Multiple Hypothesis Testing Framework for Spatial Signals

The problem of identifying regions of spatially interesting, different or adversarial behavior is inherent to many practical applications involving distributed multisensor systems. In this work, we develop a general framework stemming from multiple hypothesis testing to identify such regions. A discrete spatial grid is assumed for the monitored environment. The spatial grid points associated with different hypotheses are identified while controlling the false discovery rate at a pre-specified level. Measurements are acquired using a large-scale sensor network. We propose a novel, data-driven method to estimate local false discovery rates based on the spectral method of moments. Our method is agnostic to specific spatial propagation models of the underlying physical phenomenon. It relies on a broadly applicable density model for local summary statistics. In between sensors, locations are assigned to regions associated with different hypotheses based on interpolated local false discovery rates. The benefits of our method are illustrated by applications to spatially propagating radio waves.

==> figures/flowgraph.tex <==
\begin{tikzpicture}
	\scriptsize
	\node[coordinate] (origin) {};
	\node[coordinate, left = 0.4\textwidth of origin] (sensororigin) {};
	\node[block, anchor = center, left = .5cm of sensororigin](locCmp) {\textbf{computation of local soft decision statistic}};
	\node[input, anchor = center,  above = .175cm of locCmp] (inpData) {\textbf{local}\\\textbf{observations}};
	\node[coordinate, right = 0.35\textwidth of origin] (fcorigin) {};
	\node[block, right = 1cm of locCmp] (senLFDR) {\textbf{estimation of lfdr's at sensor locations}}; 
	\node[block, above = .175cm of senLFDR] (ipl) {\textbf{lfdr interpolation at grid points in between sensors}};
	\node[block, right = .175cm of ipl] (MHT) {\textbf{find interesting areas by making decisions for each grid point}};
	\node[sensorbox, above right=-1.1cm and -2.3cm of locCmp] {};
	\node[above = .05cm of inpData, color=black] (sensors) {\textbf{At the sensors}};
	\node[fcbox,  above right=-1.1cm and .9cm of locCmp] {};
	\node[above = .05cm of ipl, color=black] (fc) {\textbf{At the fusion center}};	

	\path[line] (inpData) -- (locCmp);

	\path[line]  (locCmp) -- (senLFDR);
	\path[line]  (senLFDR) -- (ipl);
	\path[line] (ipl) -- (MHT);
\end{tikzpicture}

==> include/ack.tex <==
% use section* for acknowledgment
\section*{Acknowledgment}
	The authors would like to thank...

==> include/bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
	Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
	Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
	Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> sections/ccl.tex <==
\section{Conclusion}
	The conclusion goes here.

==> sections/den-fit.tex <==
\section{Local false discovery rate estimation}
\label{sec:lfdr-est}
	As previously stated, the estimation of \gls{lfdr}s involves the estimation of two quantities: The null proportion $\nulFrc$ and the mixture density $\mixLocStPdf$, or instead, the alternative density $\altLocStPdf$. Since the physics of the underlying problem define the true $\mixLocStPdf$ and $\altLocStPdf$, a uniformly best approach to estimating the numerator of Eq.~\eqref{eq:lfdr-def} is impossible to determine. However, a variety of methods have been developed in the past. Most of them rely on some type of a mixture model similar to the most basic two-groups model introduced in Eq.~\eqref{eq:zval-mar-pdf_prac}. Efron himself proposed to utilize \gls{lm}, a Poisson regression technique that assumes $\mixLocStPdf$ to originate from the exponential family and estimates the model parameters using regression techniques. TODO: INSERT SOME REFERENCES.
	
	Much of recent literature focuses on estimating $\altLocStPdf$. For our problem at hand, we recommend switching back to approaches based on \pval~densities, like \cite{Pounds2003}, since in the \pval~domain, a popular approach to model $\nulPPdf$ relies on finite, parametrizable beta distribution-based mixture models, which facilitate precise modeling of the density's tail behavior.
	
	\subsection{Conservative estimation}
	\label{sec:con-est}
		In Section~\ref{sec:bfdr-lfdr}, we already emphasized that popular estimators $\nulFrcHat$ for $\nulFrc$ overestimate the true value to ensure that the resulting \gls{bfdr}\ or \gls{lfdr} estimates are not larger than the actual value. This is referred to as \textit{conservative estimation} of $\nulFrc$. However, the estimator for $\altLocStPdf$ has a similar influence on the accuracy of the \gls{lfdr} estimate.
		
		\begin{prop}
			Underestimation of the \gls{lfdr} can be caused by both, underestimation of $\nulFrc$ and overestimation of $\altLocStPdf$. While an underestimated $\nulFrc$ affects \gls{lfdr} estimates $\forall\, \locSt\in\mathbb{R}$, $\altLocStPdfHat$ must be particularly accurate in the tails of $\altLocStPdf$.
		\end{prop}
		
		\begin{proof}
			For $\lfdrHat\geq \lfdr$, $\frac{\nulFrc^2(1-\nulFrcHat)}{\nulFrcHat^2(1-\nulFrc)}\leq\frac{\altLocStPdf}{\altLocStPdfHat}$ must hold. From the right side follows, that the one-sided approximation error $\altLocStPdfHat-\altLocStPdfHat$ has to be particularly small for $\locSt$ where $\altLocStPdf$ is small.
		\end{proof}

		Since $\altLocStPdf$ and $\altLocStPdfHat$ are probability densities, underestimation $\altLocStPdfHat<\altLocStPdf\, \forall\,\locSt\in\mathbb{R}$ is impossible. Despite that overestimation of $\nulFrc$ allows to underestimate \gls{lfdr} even if $\epsilon<\altLocStPdf-\altLocStPdfHat<0$, $\epsilon\in\mathbb{R}_{<0}$, procedures that fulfill $\lfdr\, \forall\,\locSt\in\mathbb{R}$ are unnecessarily cautious to make detections. We hence define the concept of \textit{conservative \gls{lfdr} estimation} as follows.
		
		\begin{defin}[Conservative \gls{lfdr} estimators]
			\label{def:con-lfdr-est}
			If $\nulFrc < 1$, a conservative \gls{lfdr} estimator aims to provide a good estimate in the sense of $\exists\,\locSt\in\mathbb{R}: \lfdrHat<1$, while $\bfdrHat = \int_{\rejRegLocSt}\lfdrHat\leq \bfdr$ for all rejection regions $\rejRegLocSt$ of interest. A conservative \gls{lfdr} estimator is better than another conservative \gls{lfdr} estimator, if it provides the smaller value for a (potentially symmetric) distance metric of choice $d(\lfdr, \lfdrHat)$.
		\end{defin}

		\begin{prop}
			When performing multiple hypothesis testing based on \gls{lfdr} estimates, only conservative \gls{lfdr} estimators allow for detection of alternatives while strongly controlling the \gls{fdr} at nominal levels $\alpha\in[0, 1]$. 
		\end{prop}
		
		\begin{proof}
			A non-conservative \gls{lfdr} estimator could set $\nulFrcHat = 1$, regardless of the observed data. Since the resulting estimates would take values $\lfdr = 1\,\forall\locSt\in\mathbb{R}$, the \gls{fdr} would be controlled below the nominal level $\alpha\in[0, 1]$, but detections would only be made in the trivial case of $\thr = 1$. For $\thr = 1$, $\HAlt$ would be accepted $\forall\,\locSt\in\mathbb{R}$.
			
			Consider now an estimator for which $\exists\,\locSt\in\mathbb{R}:\lfdrHat<1$, but for which also $\exists\, \thr:\bfdrHat>\bfdr$. Hence, for those $\thr\in[0, 1]$ where $\bfdrHat>\bfdr$, the \gls{fdr} is not controlled at the nominal level.
		\end{proof}
		By Definition \ref{def:con-lfdr-est}, a conservative \gls{lfdr} estimator is allowed to overestimate $\lfdr$ for certain $\locSt \in\rejRegLocSt$, given that there are other $\locSt\in\rejRegLocSt$ that compensate for it. Rejection regions of interest are those subsets $\rejRegLocSt\subseteq\mathbb{R}$ to be formed when performing inference with \gls{fdr} control based on the estimated \gls{lfdr}s. Hence, for left-sided \locStval s, which we consider throughout this paper, the rejection regions of interest are $\rejRegLocSt = \rejRegZ =  (-\infty, \Phi^{-1}(\thr)]$ and $\rejRegLocSt = \rejRegP = [0, \thr]\,\forall\,\alpha\in[0, 1]$ if \zval s or \pval s are chosen, respectively. If right-sided or two-sided \locStval s were used, the rejection regions of interest would be formed using the right tails or both tails of the domain, respectively.
		
		The size of the rejection regions depend on the value of $\thr$, but they always start at the limits of the domain. Hence, precise estimation of the tails of $\altLocStPdf$ is not only required to avoid underestimation of $\lfdr$ for a single $\locSt\in\mathbb{R}$, but also to enable conservative \gls{lfdr} estimation.
	
		The concept of conservative \gls{lfdr} estimators does not allow for a universal framework to derive such optimal \gls{lfdr} estimators, since the densities under $\HAlt$ vary significantly from application to application and are often not even theoretically known. However, evaluating if a given \gls{lfdr} estimator fulfills the conditions in Definition \ref{def:con-lfdr-est} for exemplary synthetic data sets can serve to select a suitable \gls{lfdr} estimator for the application of interest.

	\subsection{Different estimation regimes}
	\label{sec:p-vs-z}
		The most popular \gls{lfdr} estimators estimate $\nulFrc$ and $\altLocStPdf$ for \zval s. Due to $\nulLocStPdf = \nulZPdf$ being a standard normal distribution, a variety of estimation schemes based on semi-parametric approaches like Gaussian deconvolution, Kernel fitting, Poisson regression, predictive recursion and Gaussian mixture models exist. TODO: INSERT SEVERAL REFERENCES.
		
		Accuracy in the tails of such estimators, which is, as we highlighted in Sec.~\ref{sec:con-est}, particularly important in \gls{lfdr} estimation, is usually difficult to obtain for a variety reasons. First, the methods usually promote an overall good fit of the estimated density to the data. Due to little probability mass in the tails, deviations there are acceptable, if the bulk if the fit in the bulk of the probability mass improves. Second, due to the lower probability mass in the tails, observing \locStval s from the tails is more unlikely. Hence, the amount of available data that provides information on the tails of the underlying \gls{pdf} is limited. Third, the domain of $\z$ stretches across the entire real axis. Hence, the support of $\altLocStPdf = \altZPdf$ and also the support of the tails, are infinitely large. 
		
		Another inconvenient problem arising when estimating the \gls{lfdr} based on \zval s is the task to split $\mixZPdf$ into the two-groups model, which includes the estimation of $\nulFrc$.
		
		The one-to-one mapping between \zval s and \pval s, $\z = \Phi^{-1}(\p)$, defines the relation between their statistical properties. The \zval~\gls{cdf} is $\mixZCdf = \mixPCdf[\Phi(\z)]$ and the \zval~\gls{pdf} is $\mixZPdf = \mixPPdf[\Phi(\z)]\phi(\z)$. 
		Estimators for \gls{lfdr} that rely on \pval s instead of \zval s exist, e.g. \cite{Pounds2003}. However, \pval-based \gls{lfdr} estimation has since lost attention, presumably due to the attractiveness of \zval s from the point of applicability of the vastly existing Gaussian theory methods \cite{Efron2010}. In contrast to the domain of the \zval s, the real axis $\mathbb{R}$, the domain of the \pval s is limited to $[0, 1]$. Hence, \pval~density estimators require more restrictive (semi-)parametric models to find a density estimate with correct support. At the same time, the limited domain of \pval s has a significant advantage: The \pval~densities do not exhibit classic distribution tails.
		
		Due to these reasons, we advocate for \gls{lfdr} estimators based on parameters estimated from \pval s instead of \zval s. 
		
		The authors of \cite{Pounds2003} proposed the popular so-called \gls{bum} model
		\begin{align}
		\label{eq:bum-def}
			\mixPPdf 	&= \nulFrc + (1-\nulFrc)\altPPdf\\
						&= \nulFrc + (1-\nulFrc)\beta(a, 1).
		\end{align}
		The \gls{bum} model is very simple and has been applied successfully in a number of applications. It also suggests $\min\mixPPdf$ as a simple estimator for $\nulFrc$. However, since the only model parameters are $\nulFrc$ and $a$, the model lacks flexibility to adjust to the data in applications where a single beta distribution is not sufficient to model the alternative \pval~density.
		
		One might resort to something one might call a multiple beta-uniform mixture model, where $\altPPdf = \sum_{\cmpIdx = 1}^{\numCmp}\altFrcLoc[\cmpIdx]\beta(a_\cmpIdx, 1)$ and $\sum_{\cmpIdx = 1}^{\numCmp}\altFrcLoc[\cmpIdx] = (1-\nulFrc)$.
		For each increment of $k$ by 1, two more parameters have to be estimated. This quickly renders the \gls{mle} approach of \cite{Pounds2003} computationally expensive, in particular, when working with large data sets. Finding \gls{mle}s for mixture models typically requires to deploy a variant of the \gls{em} algorithm TODO: INSERT REFERENCE, which is computationally demanding especially for large data sets and is at risk of finding only a locally optimal solution TODO: INSERT REFERENCE. Also, an ideal number of components $\numCmp$ has to be determined. Classic approaches for model order selection, like information theoretic criteria rely on the assumption of Gaussian distributed data and require the model to be estimated for a number of candidate models. Despite that specific \gls{itc} for beta distributed data can be derived \cite{Golz2019}, the computational burden of having to solve an already demanding, high-dimensional maximum likelihood estimation problem multiple times cannot be avoided.

		


==> sections/fd-mod.tex <==
\section{Spatial Field Model}
	\begin{itemize}
		\item Describe the data model for the spatial phenomena in general and radio waves in particular
		\item Give a couple of references to existing methods
		\item Briefly describe the model used to generate the data later used in the simulation results
	\end{itemize}

==> sections/int.tex <==
\section{Introduction}
\label{sec:int}
	The literature on methods to estimate the exact value of a spatially varying phenomenon of interest across a certain area based on spatially sparse measurements is vast and comprehensive, see, e.g., \cite{Arias2018}. While the numerical value of a specific quantity may itself be of interest, such as air temperature, precipitation or wind speed and direction when monitoring the weather, many problems require performing inferences and providing interpretations on the underlying phenomenon. Practical examples include applications in environmental monitoring (e.g. identifying regions with intolerably high emission levels), spectrum sensing (e.g. detecting regions where certain frequency bands are densely used or underutilized), smart buildings (e.g. determining areas with low oxygen levels), integrated sensing and communication (ISAC, one of the drivers of 6G wireless) or acoustics (e.g. describing the region with high ambient noise levels). %and weather monitoring.
	This fundamental problem \cite{Nowak2003} is illustrated in Fig.~\ref{fig:spa-inf}.
	
	Over the past two decades, the rapid development of ever cheaper and smaller sensors, as well as the rise of faster, lower latency and more reliable wireless connectivity standards %such as optical fiber,  5G or Bluetooth Low Energy
	have facilitated the deployment of large-scale sensor networks, a key technology in the \gls{iot}.
	% In this work, we aim to the exploit the large amount of information provided by a large-scale sensor network to infer %, within an area of interest,
	% the region in which a spatial phenomenon of interest deviates from its nominal behavior. This fundamental problem \cite{Nowak2003}
	In this work, we propose a fully data-driven framework to directly infer spatial regions of \textit{interesting}, \textit{different} or \textit{anomalous} behavior with quantitative statistical performance guarantees in terms of Type I errors using large-scale sensor networks. To this end, we model the spatial area of interest as a regular spatial grid. We formulate a \gls{mht} problem such that a decision on the state of the observed phenomenon is made at each grid point (also referred to as a \textit{location}). We discriminate between the nominal state of the phenomenon, represented by the null hypothesis $\HNul$, and any state that deviates from the nominal, represented by alternate hypotheses. While in many problems, one could distinguish various classes of {anomalous}, {interesting} or {different} behavior, we summarize everything that is not conform with the null hypothesis under the alternative $\HAlt$. \textit{Sensors} (also referred to as \textit{nodes}), capable of communicating with a cloud/\gls{fc}, are placed sparsely in distinct locations. No particular sensor distribution geometry or configuration is assumed.

	The proposed method does not presume a specific parametric spatial signal propagation model. Neither does it require raw measurements to be exchanged among neighboring nodes, nor to be transmitted to the \gls{fc}. Instead, each node communicates local information to the \gls{fc} via a scalar quantity \cite{Wang2018}. The communication of all raw measurements \cite{Arias2018} is infeasible in the context of large-scale sensor networks due to constraints on bandwidth and energy consumption \cite{Wang2018, Nitzan2020}. While the former is particularly critical when a network is composed of many agents operating in a congested spectrum, the latter is a crucial requirement for a long sensor life span.
	
	It may not be feasible to specify an accurate probability model for each node and its signal environment. The underlying probability models are learned from the data, which makes our method robust against modeling errors and suitable to a wide range of applications. However, incorporating specific models describing the underlying physics may be beneficial, as will be pointed towards the end of this paper.
	
	We propose that each node condenses its measurements in a single local sufficient statistic, likelihood ratio or \pval. Large-scale sensor networks may be composed of heterogeneous types of devices. Hence, the statistic is chosen to allow for fusing the results among potentially very different sensors. The principal purpose of dedicated emission sensors, for example, is to record data and perform inference or learning. Contrarily, smartphones equipped with a good number of different sensors collect data as a by-product of normal operation. In addition, a suitable local summary statistic is simple to compute. This limits energy consumption and reduces the hardware requirements for individual nodes. Also, it refrains from strict assumptions on the local signal model. Useful summary statistics in the \gls{mht} framework include \pval s, \zval s and (generalized) likelihood ratios. These sensor-level quantities are forwarded to the \gls{fc}, which fuses the information to identify the local regions associated with different hypotheses.
%	An algorithm is suitable to work with a large quantity of data, if it is capable to extract information in a computationally efficient manner. In addition, it should also be capable to compensate for differences and limited comparability of individual data points, since large-scale sensor networks may be composed of various types of devices. For some, like dedicated emission sensors, the recording of data is the principal task, while others, such as cellphones, gather them as a byproduct. The type and quality of the collected data vary from sensor to sensor and communication with the {cloud} is limited due to bandwidth and energy consumption constraints. Thus, continuously streaming raw data to the cloud seems infeasible \cite{Arias2018}.
%	We propose to treat the aforementioned task as a \gls{mht} problem, so that a binary decision on the state of the observed phenomenon is to be made at each point on a regular grid of locations. At each location, one decides between the nominal state of the phenomenon, represented by the null hypothesis $\HNul$, and anomalous behavior, indicated by the alternative $\HAlt$. In what follows, we will refer to the entirety of locations points at which $\HNul$ ($\HAlt$) is in place as the \textit{null} (\textit{alternative}) region. By embedding the problem into the framework of hypothesis testing, we are able to provide statistical performance guarantees on the spatial accuracy of the identified alternative regions. The scalability to large-scale sensor networks is ensured by condensing the raw data at each individual sensor into a simple local summary statistic, which expresses the sensor's trust in observing the nominal state of the phenomenon. Prime examples include \pval s, \zval s or likelihood ratios. These local statistics are forwarded to a \gls{fc} that identifies the null and alternative regions by the joint evaluation of all local summary statistics.
	Our work differs from distributed inference \cite{Veeravalli2012}, where a single binary decision on the state of the phenomenon across the {entire} area is made.
	
	In dependence on the size of the monitored area and the desired spatial resolution, the number of grid points and hence decisions might easily reach
	%Since the goal is to precisely locate the areas of anomalous behavior, the spatial grid is a fine partition of the monitored area and the number of decisions might easily reach
	the order of tens of thousands. To prevent a flood of false positives by testing for $\HNul$ a large number of times \cite{Tukey1991}, we follow the principles of \gls{mht}, where %The principles of \gls{mht} are to be applied to guard against a flood of false positives \cite{Tukey1991}, caused by testing $\HNul$ a large number of times.
	choosing the alternative $\HAlt$ is called a \textit{discovery} \cite{Soric1989}. Performance guarantees are commonly provided w.r.t. the \gls{fdr}, which is the expected proportion of false discoveries among all discoveries,  \cite{Benjamini1995}.
	Controlling the \gls{fdr} is similarly popular to constraining the false alarm probability in binary hypothesis testing. When the number of true positives increases, procedures that control the \gls{fdr} allow more false positives than classic \gls{mht} methods applied, e.g., in \cite{Zoubir1995}. Thus, controlling the \gls{fdr} leads to a larger detection power. % Such behavior is acceptable in a broad range of applications \cite{Benjamini2010}.  %Consequently, the \gls{fdr} is controlled by incorporating all available information into the determination of a threshold for the deployed test statistic, which results in a larger detection power than a pure correction of the threshold for the number of times $\HNul$ is tested \cite{Benjamini1995}.
	
	Attempting to control the \gls{fdr} in our spatial inference setup poses the following problem-specific challenges. First, local summary statistics are only available at the subset of grid points where the sensors are located, but decisions between $\HNul$ and $\HAlt$ need to be made at every grid point. Second, the deployed method must scale well to large-scale sensor networks, i.e., its computational complexity remains moderate even for a large number of nodes. Finally, the method should allow for incorporating available side information into the decision process to increase the detection power.
	
	The past work on \gls{fdr} control in the context of spatial data has focused on testing a priori \cite{Benjamini2007, Barber2015a} or a posteriori \cite{Chouldechova2014, Chumbley2009, Chumbley2010, Schwartzman2019} formed groups of data. While these procedures typically rely on assumptions that may not be realistic \cite{Eklund2016}, they do also not provide guarantees w.r.t. to the localization accuracy of the identified alternative area. Random field-based approaches like \cite{Sun2014, Shu2015} suffer from excessive computational cost if the number of nodes is large. 
	We find the concept of the \gls{lfdr} \cite{Efron2001, Efron2005, Efron2008, Efron2010} particularly suitable to deal with the aforementioned challenges. The \gls{lfdr} is computed for each sensor and quantifies the risk of making a false discovery when accepting $\HAlt$ at its location. %The \gls{lfdr} can also be interpreted as the empirical Bayes posterior probability of $\HAlt$ \cite{Efron2010}.
	Previous work \cite{Efron2010, Tansey2018, Halme2019, Golz2019, Scott2015, Chen2019} demonstrates its capability to incorporate available side information like spatial proximity into decision making.
	
%	The control of the \gls{fdr} in the context of spatial data has been subject to research since \cite{Pacifico2004}, often in the context of \gls{fmri}. Much of the previous work is dedicated to controlling the \gls{fdr} not for individual data points, but for grouped data. Regardless of whether the groups are formed \textit{a priori} \cite{Benjamini2007, Barber2015a} or based on the data \cite{Chouldechova2014, Chumbley2009, Chumbley2010, Schwartzman2019}, such group-level control does not allow to assess the spatial accuracy of the detected alternative region. %A true positive = signal somewhere within the group
%	Also, these procedures typically require a set of restrictive assumptions on the statistical behavior of the underlying phenomenon, which are difficult to establish in practice \cite{Eklund2016}.
%	
%	The concept of the \gls{lfdr} \cite{Efron2001, Efron2005, Efron2008, Efron2010} is particularly suitable to our problem, since it allows to incorporate covariate information like spatial proximity into the decision process \cite{Efron2010, Tansey2018, Halme2019, Golz2019}. Computed individually for each decision between $\HNul$ and $\HAlt$, the \gls{lfdr} quantifies the risk making a false discovery when accepting $\HAlt$ for this test. Once the \gls{lfdr}'s have been computed, \gls{fdr}-controlled identification of the alternative region is straight forward. Moreover, the \gls{lfdr} is an attractive soft decision statistic, since it can be interpreted as the empirical Bayes posterior probability of $\HAlt$ \cite{Efron2010}.
	
	The \gls{lfdr}'s are computed from the local summary statistics. In addition, the \gls{lfdr}'s rely on the joint \gls{pdf} of the local summary statistics and the overall proportion of alternatives that are unknown in practice. These quantities need to be learned or estimated accurately from the data. This is often referred to as \textit{\gls{lfdr} estimation} in the \gls{mht} literature \cite{Efron2010}.	%\Gls{lfdr}s rely on the local summary statistics as well as on the - in practice estimated - proportion of true alternatives and the joint \gls{pdf} of the local statistics.
	A variety of estimators exist, often assuming that the joint \gls{pdf} belongs to the exponential family \cite{Efron2010, Muralidharan2010, Martin2011, Scott2015}.
%	The vast literature on spatial \gls{mht} in the context of biomedical imaging does not fear computational complexity of the applied methodology, since resources as time and hardware are often not tightly restricted. Yet, scalability issues have been reported on methods like \cite{Sun2014, Shu2015}.
%	On the contrary, easiness on resources is of fundamental importance in our application. The prerequisite in order to apply methods that take into account spatial information to increase detection power is hence an efficient method to accurately determine \gls{lfdr}'s in the first place.
	Our novel contributions in this work are as follows. 
	\begin{itemize}
		\item We formulate an \gls{lfdr}-based framework as a flexible data-driven approach to accurately determine spatial regions of interest, difference or anomaly of a physical phenomenon. %Second, we introduce the principle of conservative \gls{lfdr} estimation to explain violations of the nominal \gls{fdr} level observed when applying existing \gls{lfdr} estimation methods in Sec.~\ref{sec:lfdr-est-gen}. 
		\item We propose a novel, highly computationally efficient method for computing \gls{lfdr}'s. It bases upon an innovative mixture distribution model and the method of moments.
		\item We demonstrate that proper interpolation of the \gls{lfdr}'s between sensors allows for inferring the state of the phenomenon even at locations between the sensors, where measurements are unavailable. Our proposed method scales well to spatial inference with large-scale sensor networks under strict statistical performance guarantees.
	\end{itemize}
 %The simulation results in Sec.~\ref{sec:sim-res} illustrate the functionality of the proposed method.
%	Our contributions in this work are as follows. First, we establish the spatial inference model as a framework to precisely localize the region of anomaly of an observed physical phenomenon in an area of interest. Second, we introduce the principle of conservative \gls{lfdr} estimation. Third, we propose a very fast and effective method for computing \gls{lfdr}'s, based on a beta distribution mixture model and the \gls{mom}. Fourth, we discuss, how to identify the alternative region when data are available only for a sparse subset of locations. 

%	\begin{figure}
%		PLACEHOLDER
%		\caption{Illustration}
%		\label{fig:intro}
%	\end{figure}


==> sections/ipl.tex <==
\section{Interpolation}
\label{sec:ipl}
	TODO: Description of radio field
	\begin{itemize}
		\item give important equations
		\item describe what can be neglected (fast-fading)
	\end{itemize}
	TODO: Brief summary on REM estimation
	\begin{itemize}
		\item including the justification why parameteric radio field estimation (aka, estimating the location of the source followed by estimation of the shadow fading) is typically not done (cite relevant literature)
	\end{itemize}
	\subsection{Hypothesis testing on interpolated data}
		TODO: Descrribe why neither binary nor multiple hypothesis testing work out of the box for interpolated data
		\begin{itemize}
			\item distribution of interpolated statistics changes
			\item give an example
			\item mention empirical null estimation by Efron, but also tell that it requires a large fraction of true nulls greater than $90\%$ among all tested hypotheses
		\end{itemize}



==> sections/lfdr-est.tex <==
\section{The proposed \gls{lfdr} estimator}
	\label{sec:lfdr-est}
	In this section, we incorporate the previously developed \gls{smom} estimator for spherically beta distributed data into an efficient \gls{lfdr} estimation algorithm. The simulation results in Sec.~\ref{sec:sim-res} suggest that this \gls{lfdr} estimator is conservative in the sense of Definition~\ref{def:con-lfdr-est}, while being more powerful than existing methods for a variety of scenarios.
	
	The idea of large-scale inference, to \textit{learn from the experience of others} \cite{Efron2010} allows to treat the input data $\pSetPx = \{\p[1], \dots, \p[\numPx]\}$ as $\numPx$ realizations of a single same random variable $\p[]\sim\mixPPdf$. Traditional techniques would treat $\pSetPx$ as a single observation of a $\numPx$-dimensional random vector instead. 
 	We propose to partition the observation data $\pSetPx$ into $\numTls= \lfloor\numPx/\numVecEl\rfloor$ subsets $\mathcal{P}^{\numVecEl}_1, \dots, \mathcal{P}^\numVecEl_{\numTls}$ of dimension $\numVecEl$ and estimate $\mixPPdf$, based on a multivariate density fit, followed by marginalization. To the best of our knowledge, such a concept is entirely new to \gls{lfdr} estimation.
 
	\subsection{Multivariate p-value density estimation}
		In this work, we observe a physical phenomenon on a continuous spatial area. In practice, this area is discretized into a regular grid of $\numPx$ smallest spatial units, so-called\text{pixels}. Additionally, subdividing the observation area into larger units comprising more than a single atom seems intuitively reasonable. Hence, we propose to form the mutually exclusive subsets, $\tlIdx\in[\numTls]$,
		\begin{align}
			\mathcal{P}^{\numVecEl}_\tlIdx = \bigg\{\pPx\Big|\pxIdx&:\sqrt{\numVecEl}\Big(\tlIdx-1-\numPxX\Big\lfloor\frac{\tlIdx\sqrt{\numVecEl}}{\numPxX+1}\Big\rfloor\Big)+1\leq\xPx\nonumber\\
			&\quad\leq\sqrt{\numVecEl}\Big(\tlIdx-\numPxX\Big\lfloor\frac{\tlIdx\sqrt{\numVecEl}}{\numPxX+1}\Big\rfloor\Big), 		\label{eq:tiles}\\ &\Big\lfloor\frac{\tlIdx\sqrt{\numVecEl}}{\numPxX+1}\Big\rfloor\sqrt{\numVecEl}+1\leq \yPx\leq \Big(\Big\lfloor\frac{\tlIdx\sqrt{\numVecEl}}{\numPxX+1}+1\Big\rfloor\sqrt{\numVecEl}\Big)\bigg\}\nonumber,
		\end{align}
		i.e., such that squares of $\numVecEl$ neighboring pixels are comprised in \textit{tiles} to form a regular grid across the observation region. $\numPxX$ and $\numPxY$ denote the $\x$ and $\y$ dimensions of the observed area, i.e., $\numPx = \numPxX\numPxY$. Also, $\{\numVecEl \in\mathbb{N}|\sqrt{\numVecEl}\in\mathbb{N}\}$.
		
		Formally, define a random vector $\pvec \in\mathbb{R}^{\numVecEl} \sim\mulPPdfMix$ with observation set $\pMulSetPx = \{\pvec_{1}, \dots, \pvec_{\numTls}\}$. We model $\mulPPdfMix$ by
		\begin{equation}
			\label{eq:mulvar-p-mix-dens}
			\mulPPdfMix = \sum_{\cmpIdx = 1}^{\numCmp}\cmpWgt\mulPPdfCmp{\cmpIdx},
		\end{equation}
		a multivariate mixture model with $\numCmp$ components. In practice, we expect a small $\numCmp$ to be sufficient for efficient approximation of the underlying true probability model, since a few, distinct classes of tiles should suffice to explain the statistical behavior of the data. Namely, some tiles close to sources will be composed of pixels that all are heavily under the influence of the observed spatial phenomenon, whereas tiles located further away might be composed of both, pixels at which $\HNul$ is in place and pixels at which $\HAlt$ is in place. Additionally, tiles where $\HNul$ holds for all pixels are expected to arise in locations far away from any source.
		
		We propose to extend the \gls{bum} model from Eq.~\eqref{eq:bum-def}, to the multivariate data model by designing a multivariate mixture of element-wise single-parameter beta distributions for $\mulPPdfMix$. Under the assumption that the elements $\p[\vecElIdx], \vecElIdx\in[\numVecEl]$ are independently distributed random variables, we define
		\begin{equation}
			\label{eq:mulvar-beta-model}
			\p[\vecElIdx] \sim \sum_{\cmpIdx = 1}^\numCmp\cmpWgt\mathrm{beta}\Big(\betaMixA, 1\Big),\qquad \forall\,\vecElIdx\in[\numVecEl]
		\end{equation}
		for the entries of $\pvec = [\p[1],\dots, \p[\numVecEl]]^\top$. Unlike the \gls{bum} model, Eq.~\eqref{eq:mulvar-beta-model} does not contain an explicit null component. However, since the uniform distribution is equivalent to $\mathrm{beta}(1, 1)$, any appropriate density estimator will recover the null component as one of the $\numCmp$ mixture components.

		By marginalization, we obtain
		\begin{equation}
			\label{eq:prop-p-dens-mod}
			\mixPPdf = \frac{1}{\numVecEl}\sum_{\cmpIdx = 1}^\numCmp\cmpWgt\Bigg(\sum_{\vecElIdx= 1}^\numVecEl\mathrm{beta}\Big(\betaMixA, 1\Big)\Bigg).
		\end{equation}
		Let us briefly emphasize some advantages of the model in Eq.~\eqref{eq:prop-p-dens-mod} over the one in Eq.~\eqref{eq:bum-def}. First, it offers greater flexibility due to $\numCmp(1+\numVecEl)$ tunable parameters instead of two. Second, summarizing pixels in tiles enforces structure an intuitive structure on the mixture components, most notably expressed by having $\numCmp\numVecEl$ mixture components but only $\numCmp$ mixture weights. This structure comes natural for spatial data and will result in more stable density models than if one was to simply design the mixture by a regular one-dimensional single-parameter beta mixture with $\numCmp(1+\numVecEl)$ components and component weights. Third, the introduction of tiles allows the application of multivariate density estimation techniques such as the fast and efficient method from Sec.~\ref{sec:sMoM}. 
		
		Mixture models composed of a potentially large number components are particularly hostile to maximum likelihood estimation, as the high-dimensional optimization function is in general highly non-convex with a lot of local optima. Simultaneously, the computational complexity of the typically deployed \gls{em}-based estimation procedures does not only increase rapidly in the number of model parameters, but also in the number of available observations.
		
		In contrast, the \gls{mom} provides better estimates the more data is available, while the computational complexity only depends on the model. For certain specific data models, the problematic dependency of the method of moments on unstable higher order moments can be circumvented by techniques like the spectral method of moments from Sec.~\ref{sec:sMoM}. In what follows, we will motivate the application of the \gls{smom} to our problem.

	\subsection{Applicability of \learnSB~to \pval~density estimation}
		\learnSB~ relies on two central assumptions, besides that the entries of the multivariate random vector $\pvec$ each must follow a beta mixture distribution.
		
		Condition~\ref{cond:1} requires, per component, distinct values for the $\numVecEl$ means of the random vector entries. We work with quantities estimated from the observed data. Consequently, the sample means differ with probability $1$, even if the element-wise population component means are equivalent.
		
		The spherical covariance assumption appears to be a unjustified at first glance. This assumption would be enforced if for a particular $\cmpIdx\in[\numCmp]$, $\betaMixA\,\forall\,\vecElIdx\in[\numVecEl]$ were derived from the estimated component variances $\cmpVarEst$, which would lead to identical $\betaMixA\,\forall\,\vecElIdx\in[\numVecEl]$. In addition, it would imply that the \pval s of pixels within the same tile are identically distributed. As previously outlined, we explicitly expect tiles to be composed of both, pixels at which $\HAlt$ and pixels at which $\HNul$ is in place. Hence, assuming identical distributions for all pixels within a tile is fairly unrealistic. Fortunately, the model in Eq.~\ref{eq:prop-p-dens-mod} is composed of single-parameter beta distribution components and we can estimate the required $\cmpWgt$ and $\betaMixA$, $\forall\,\cmpIdx\in[\numCmp]$ and $\forall\,\vecElIdx\in[\numVecEl]$ exclusively based on the estimated component mean vectors $\vecCmpExpEst$.

		Of course, the spherical covariance assumption is present in \learnSB~also without explicit enforcement. Yet, the procedure remains applicable as long as the component variances $\cmpVarEst, \cmpIdx\in[\numCmp]$ are close to the true element-wise variances $\mathrm{var}_{|\cmpIdx}(\p[\vecElIdx]), \forall\,\vecElIdx\in[\numVecEl]$ conditioned on mixture component $\cmpIdx\in[\numCmp]$, which allows those to be \textit{similar but not necessarily identical}. The latter is a reasonable assumption: Spatial phenomena typically vary smoothly across the spatial domain and since the tiles are composed of closely-located pixels, similar but not necessarily identical statistical properties at pixels within a tile are realistic. We conclude that Alg.~\ref{alg:learnSB} is suitable to estimate the model parameters for Eq.~\eqref{eq:mulvar-p-mix-dens}.

	\subsection{Proposed algorithm}
		Our proposed \gls{lfdr} estimator is summarized in Alg.~\ref{alg:spa-lfdr-est}. In brief, the algorithm operates by running the previously developed \gls{smom} several times on the tiled \pval s. In each run, the \pval s from the same tile are sorted differently at random within the tile vector. This is repeated for a couple of candidate model orders $\candNumCmp = 1, 2, 3, \dots$ and candidate tile sizes $\candNumVecEl = 4, 9, 16, \dots$, where the former are required to be positive integers and the latter positive integers with an integer square root.
		
		The multiple runs with differently sorted tile vectors are required since we aim to assign two tiles composed of similarly behaved \pval s to the same component $\cmpIdx$, regardless of the position of the corresponding pixes within the tile. Consider, for example, two $2\times2$ tiles. Say, both contain three pixels and one pixel at which $\HNul$ and $\HAlt$ are in place. Also, $\HAlt$ leads to statistically similarly behaving alternate \pval s in both tiles. However, for the first tile, $\HAlt$ is in place at the pixel located in the top left corner, whereas in the second, $\HAlt$ is in place at the pixel located in the bottom right corner. If the ordering of the entries of the tile vectors depended on the location of pixels within the tile, associating those two tiles the same mixture model component would not be justified.
		
		\begin{algorithm}
			\caption{Proposed \gls{lfdr} estimator for spatial data}
			\label{alg:spa-lfdr-est}
			\hspace*{\algorithmicindent} \textbf{Input}: $\pSetPx = \{\p[1], \dots, \p[\numPx]\}$, $\candNumCmp$, $\candNumVecEl$, $\numPer$, $\numPxX$, $\numPxY$, $\disFct{\cdot}{\cdot}$\\
			\hspace*{\algorithmicindent} \textbf{Output}: $\lfdrHat[{\p[1]}], \dots, \lfdrHat[{\p[\numPx]}]$
			\begin{algorithmic}[1]
				\vspace{1pt}
				\Statex\textbf{Step 1:} \textit{Estimation of $\mixPPdf$}
				\State Initialize $\disMsr = \infty$
				\State Compute the histogram $\pHist$ for the data in $\pSetPx$
				\For{$\numVecEl\in\candNumVecEl$}
					\State Divide $\pSetPx$ into the tile sets $\mathcal{P}^{\numVecEl}_\tlIdx$, $\tlIdx \in[\numTls]$
					\For{$\perIdx\in[\numPer]$}
						\State Form vectors $\pvec_\tlIdx\in\mathbb{R}^{\numVecEl}, \forall\,\tlIdx\in[\numTls]$, by random ordering of the elements in $\mathcal{P}^{\numVecEl}_\tlIdx$
						\State Form $\pvecSet^\numTls = \big\{\pvec_{\tlIdx}\in\mathbb{R}^{\numVecEl}\,|\,\tlIdx\in[\numTls] \big\}$
						\For{$\numCmp\in\candNumCmp$}
							\State Find $\cmpWgtEst$, $\betaMixAEst, \forall\,\cmpIdx\in[\numCmp], \forall\,\vecElIdx\in[\numVecEl]$ via Alg.~\ref{alg:learnSB}
							\State Insert $\cmpWgtEst$, $\betaMixAEst$ into Eq.~\eqref{eq:prop-p-dens-mod} to obtain $\mixPPdfEst$
							\If{$\disFct{\pHist}{\mixPPdfEst}<\ell$}
								\State $\disMsr = \disFct{\pHist}{\mixPPdfEst}$, $\optMixPPdfEst = \mixPPdfEst$
							\EndIf 
						\EndFor
					\EndFor
				\EndFor
				\vspace{3pt}
				\Statex \textbf{Step 2:} \textit{Estimation of $\nulFrc$ and $\altPPdf$}
				\State Compute $\nulFrcHat = \min\big(\optMixPPdfEst\big)$
				\State Compute $\altPPdfEst = \big(1-\nulFrcHat\big)^{-1}(\optMixPPdfEst-\nulFrcHat\big)$
				\State Determine $\lfdrHat[\pPx], \forall\,\pxIdx\in[\numPx]$ from Eq.~\eqref{eq:lfdr-def} using $\nulFrcHat$, $\altPPdfEst$
			\end{algorithmic}
		\end{algorithm}
	
		Alg.~\ref{alg:spa-lfdr-est} selects the best model estimate based on the random data permutation and model parameters $\numCmp$ and $\numVecEl$ in the sense of minimizing a pre-specified distance measure $\disFct{\mixPPdfEst}{\pHist}$ between model estimate $\mixPPdfEst$ and the histogram of the observed data. We ran Alg.~\ref{alg:spa-lfdr-est} with some of the most popular measures for quantifying closeness based on probability densities and distribution functions. We found Alg.~\ref{alg:spa-lfdr-est} to be robust w.r.t. the selected distance measure, no significant differences were observed for \gls{kld}, \gls{wsd}, \gls{jsd} or \gls{ksd}.
		
		In Sec.~\ref{sec:sMoM_theo-pop-mom-rel}, we stated that the relations exploited in the derivations of \learnSB~rely on large $\numVecEl$ for spherically beta distributed data. However, in Alg.~\ref{alg:spa-lfdr-est}, an increase in the size of the tiles $\numVecEl$, reduces the number of available realizations $\numTls$. Accounting for this trade-off through determination of an analytically optimal $\numVecEl$ appears to be tedious and unnecessary, since selecting the model that fits best to the data produces very good results.
		
		The same applies to the model order $\numCmp$. %Note that classic model order selection problems differ from our model in Eq.~\eqref{eq:prop-p-dens-mod}, since we add $\numVecEl$ model components per smallest increment of the model order $\numCmp$.
		To avoid overfitting, one traditionally determines the model order by either \gls{itc} or hypothesis testing based approaches. Our proposed \gls{lfdr} estimator, in contrast, is not at risk of overestimating the model order. To this end, observe that Eq.~\ref{eq:prop-p-dens-mod} does not contain an explicit uniform component representing the \pval s originating in $\HNul$. Thus, at least one of the estimated $\numCmp$ mixture components majorly represent $\HNul$. %In practical cases of interest, the null proportion $\nulFrc$ is fairly large, making the null component the pre-dominant mixture component.
		and inevitably, as $\numCmp$ grows, a point will be reached beyond which more than a single component will represent \pval s from pixels at which $\HNul$ is in place. Single-parameter beta distribution mixtures are fairly inflexible when it comes to modeling a uniform distribution such that even an infinite mixture $\lim\limits_{\numCmp\rightarrow\infty}\sum_{\cmpIdx = 1}^\numCmp \cmpWgt\mathrm{beta}(\betaMixA, 1)$ with model parameters $\betaMixA\neq 1$ provides a worse fit than a single $\mathrm{beta}(1, 1)$. This is different from Gaussian mixture models, which provide the best fit to any data when the number of mixture components is equivalent to the number of data points with component variances going to zero. Due to this difference, the quality of estimates based on Eq.~\eqref{eq:prop-p-dens-mod} deteriorates as soon as increasing $\numCmp$ only increases the number of components modeling the null part of $\mixPPdf$, thereby preventing model overfitting.
		
		As a final remark on Alg.~\ref{alg:spa-lfdr-est}, we highlight that we apply a slightly modified version of \learnSB. Namely, in line 4 of Alg.~\ref{alg:learnSB}, we estimate $\avVarEstSet{\mathcal{S}}$ not by the $\numCmp$-th largest, but by the smallest eigenvalue of ${}_{\mathcal{S}}\hat{\vecCov}$ to avoid overestimation of the noise variance, since such this would pose a potential risk of missing out on non-noise contributions by mixture components with small, but non-zero variance.

==> sections/lfdr.tex <==
\section{Local False Discovery Rates}
	\label{sec:lfdr}

==> sections/mul-hyp.tex <==
\section{Multiple Hypothesis Testing}
\label{sec:mul-hyp}
TODO: Write about local decision statistics
\begin{itemize}
	\item likelihood ratio tests
	\item Neyman-Pearson test
	\item \pval~thresholding
	\item (semi)-parametric vs. non-parametric tests
	\item sequential tests
	\item etc.
\end{itemize}
TODO: Write what is always needed - at least a test statistic and its distribution under the null, distribution under the alternative as optional feature to increase power\\
\begin{itemize}
	\item null distribution either analytically determined or by empirical methods (e.g. bootstrap)
\end{itemize}
TODO: Cite work on hypothesis testing relevant to spectrum sensing\\
TODO: Introduce \pval s and \zval s as local decision statistics
\begin{itemize}
	\item soft local decisions (in contrast to hard binary decisions)
	\item \pval~and\zval~can basically always be obtained
	\item each sensor can operate independently of others
	\item sensors can be totally different from each other
\end{itemize}
TODO: Why do we need multiple testing correction
\begin{itemize}
	\item justify why false alarm probability is not meaningful when testing multiple times
	\item give an example - maybe also relate to current corona testing
\end{itemize}
TODO: Formally introduce FDR and so on\\
TODO: Raise issues with multiple testing: low detection power\\
\begin{itemize}
	\item but this is a price one has to pay, as single test false alarm probabilities are not meaningful
\end{itemize}
	\subsection{Spatial Inference}
		TODO: Describe smoothness of spatial fields\\
		TODO: Introduction to multiple hypothesis testing in the spatial context
		\begin{itemize}
			\item the two-groups model (marginal and local)
			\item Bayesian FDR
		\end{itemize} 
		TODO: Brief overview on existing approaches in spatial multiple hypothesis testing, including a general motivation (increase in detection power)
		\begin{itemize}
			\item weighted approaches?
			\item Gaussian field-based approach
			\item local variation of the null prior
			\begin{itemize}
				\item original idea by Efron
				\item our own approach (clustering-based)/Topis approach
				\item highlight, that small priors are particularly needed for sensors "on the edge" of the detection region -> typically really difficult to obtain
				\begin{itemize}
					\item proof this by my "local oracle" example
				\end{itemize}
			\end{itemize}
			\item smoothing-based approaches
			\begin{itemize}
				\item Stating that smoothing is similar to increasing the SNR of the local statistics
				\item p-value smoothing -> Comparison to z-score smoothing, based on Efron, show that this is superior
			\end{itemize}
		\end{itemize}

%Spatial smoothness is a common property of many real-world phenomena. Typically, large signal values $\sig$ occur at locations $\crd$ close to each other and the sets $\setFdNul$ and $\setFdAlt$ are composed of spatially homogeneous regions. A radio field, for example, is characterized by high signal values close to the transmitter and a decrease in signal strength with increasing distance. Of course, not only a single but $\numEv$ transmitters might be present within the observation scope of the field $\setFd$. Generally speaking, the null hypothesis might be violated in $\numEv$ spatially homogeneous regions due to $\numEv$ anomalous events, each of them causing independent homogeneous regions of anomaly $\evFd$, $\evIdx = 1, \dots, \numEv$, with their union $\setFdAlt = \bigcup_{\evIdx = 1}^{\numEv}\evFd$. We will exploit spatial smoothness later on to increase detection power 

%The local decision between $\HNul$ and $\HAlt$ is typically made based on a sufficient statistic, that can be (semi-)parametric such as a \gls{glr} [INSERT RELEVANT CITATION W.R.T. SPECTRUM SENSING] or non-parametric, such as the signal energy [INSERT RELEVANT CITATION W.R.T. SPECTRUM SENSING].
 


==> sections/pro-for.tex <==
\section{Problem Formulation}
\label{sec:pro-for}
	In this section, we provide a general mathematical formulation of the considered problem and introduce some basic notation that will be used throughout the remainder of this work.

	We aim to identify spatial regions of anomaly, in which a phenomenon of interest behaves differently than expected. Define a spatial field by $\spaFdSym: \setFd \mapsto \mathbb{C}$, by assigning a field value $\spaFd$ to each coordinate vector $\crd \in \setFd \subseteq \mathbb{R}^\spaDim$, where $\setFd$ denotes the spatial region over which the field is monitored. In what follows, $\spaDim = 2$, since many real-world phenomena are typically modeled as two-dimensional spatial fields.
	We assume an additive field model
	\begin{equation}
	\label{eq:add-fd-mod}
		\spaFd = \sig + \noiSpa,
	\end{equation} 
	where $\sig$ and $\noiSpa$ are signal and noise at location $\crd$, respectively.

	In a radio spatial field, this model could represent the signal received at a mobile user in a certain frequency band. If no transmitter is active, the user would only observe noise.

	\Gls{wlog}, we define the problem of distinguishing between nominal and anomalous state at $\crd$ as a binary decision problem with a simple null hypothesis $\HNul$ representing the nominal state of the field and a composite alternative $\HAlt$, i.e.,
	\begin{equation}
	\label{eq:hyp-def}
		\begin{aligned}
			\HFd = \HNul: \qquad &\sig = 0,\\
			\HFd = \HAlt: \qquad &\sig \neq 0,
		\end{aligned}
	\end{equation}
	where $\HFd$ is the true field state at location $\crd$.  We can now define two mutually exclusive sets $\setFdNul = \{\crd\,|\, \HFd = \HNul\}$ and $\setFdAlt = \{\crd\,|\,\HFd=\HAlt\}$.

	The set $\setFd$ is a continuous space and hence contains infinitely many elements. In practice, we cannot test at infinitely many locations $\crd$. Therefore, we follow the common procedure of discretizing the support of the spatial field by a grid of pixels when $\spaDim = 2$. The discrete quantities corresponding to $\setFd$, $\setFdNul\subseteq\setFd$ and $\setFdAlt = \setFd \setminus \setFdNul$ shall be denoted by $\setPx\subset\setFd$, $\setPxNul\subseteq\setPx$ and $\setPxAlt = \setPx \setminus \setPxNul$, respectively. Assuming a total number of $\numPx = \left|\setPx\right|$ locations in the region of interest, we will denote the corresponding coordinate vectors by $\crdPx$, $\pxIdx = 1, \dots, \numPx$ and corresponding field values by $\spaFd[\crdPx]$ in what follows. The larger $\numPx$, the higher the spatial resolution.

	In this work, we consider the monitoring of spatial fields by large-scale sensor networks. The assumption that field measurements $\spaFd[\crdPx]$ can be obtained $\forall\,\crdPx \in \setPx$ is practically infeasible. Sensor networks should rather be interpreted as a set $\setSen$ of sampling locations $\crdSen$, $\senIdx = 1, \dots, \numSen$ that are spatially sparse and in general non-homogeneously distributed, with the number of sensors $\numSen = \left|\setSen\right|\ll \numPx$. Regardless, conclusions about the state of the field at every \textit{pixel} $\crdPx$ are to be drawn. In other words, we are looking to separate $\setPx$ into $\setPxNul = \left\{\crdPx\, |\,\HPx = \HAlt\right\}$ and $\setPxAlt = \left\{\crdPx\,|\,\HPx = \HNul\right\}$ given noisy measurements $\spaFd[\crdSen]$ $\forall\,\crdSen\in \setSen$, where $\setSen \subseteq \setPx$. By all means, performance guarantees in terms of meaningful error measures are to be given. We will elaborate on that in the following section.
	

==> sections/pro-met.tex <==
\section{Proposed Method}
\label{sec:pro-met}
	TODO: Justify the use of Delaunay triangulation
	\begin{itemize}
		\item also bring in some performance comparison from previous work with Kriging, showing, to quantify how much better Kriging performs 
	\end{itemize}
	TODO: Connect the smoothing with the interpolation\\
	TODO: Proof Positive regression dependency on a subset condition for interpolated data\\
	TODO: Highlight, that besides the smoothing property of interpolation, there are now locally varying null distributions of the z-scores
	\begin{itemize}
		\item different from existing methods, none of them assumes locally varying null distributions for the \zval s, even though this option was mentioned by Efron
		\item 
	\end{itemize}
	TODO: Describe our proposed method in detail
	\begin{itemize}
		\item interpolation strategy, along justifications
		\begin{itemize}
			\item affine invariance
			\item computational simplicity
			\item well-established properties of interpolated values
		\end{itemize}
		\item derivation of the null distribution of z-scores of interpolated data
		\item subsequently apply false discovery rate smoothing
		\begin{itemize}
			\item if local distributions not computable, use globals
		\end{itemize} 
	\end{itemize}
	TODO: Different versions of Delaunay triangulation
	\begin{itemize}
		\item "normal"
		\item with constraints that create a continuously differentiable field
	\end{itemize}

==> sections/sMoM.tex <==
\section{The spectral method of moments}
	\label{sec:sMoM}
	In this section we propose a novel approach to estimating the \pval~\gls{pdf} $\mixPPdf$ based on a recently developed variation \cite{Anandkumar2012, Hsu2012} of Pearson's \gls{mom} \cite{Pearson1936}. The \gls{mom} matches the moments of the observed data to the theoretical population moments. In contrast to \gls{mle}s, \gls{mom} estimators have in general a low computational complexity.
	
	The standard \gls{mom} estimates one moment per unknown parameter. Since higher order moment estimators exhibit large variance, applying the classic method of moments for parametric models with many model parameters may lead to inaccurate estimates.
	The \gls{smom} framework circumvents this problem for multivariate data by estimating the mixture model parameters exclusively from the first three moments.

	In this work, we extend the method for estimating the parameters of spherical multivariate Gaussian mixture models introduced in \cite{Hsu2012} to spherically multivariate beta distributed data under certain conditions. As discussed in Sec.~\ref{sec:con-est}, conservative \gls{lfdr} estimation requires estimation accuracy in particular in the tails of $\altZPdf$, which is the reason we recommended to estimate \gls{lfdr}s based on \pval s rather than on \zval s in Sec.~\ref{sec:p-vs-z}. The \gls{pdf} of \pval s are commonly modeled by beta distributions. Sec.~\ref{sec:lfdr-est} contains our proposed fast and efficient algorithm for \gls{lfdr} estimation.
	
	\subsection{Multivariate spherically beta distributed data}
	\label{sec:sMoM_mv-sph-beta-data}
		Consider a $\numVecEl\times 1$ multivariate random vector $\pvec = [\p[1], \dots, \p[\numVecEl]]^\top$ with $\p[\vecElIdx] \sim \sum_{\cmpIdx = 1}^{\numCmp}\cmpWgt\cdot\mathrm{beta}\Big(\betaMixA, \betaMixB\Big)$ and weight vector $\cmpWgtVec = \big[\cmpWgt[1], \dots, \cmpWgt[\numCmp]\big]^\top$ with $\sum_{\cmpIdx = 1}^\numCmp \cmpWgt = 1$. The $\p[\vecElIdx]\,\forall\,\vecElIdx\in[\numVecEl]$ are independently distributed. %The distributions of the random vector entries are hence mixtures of beta distributions with $\numCmp$ mixture components.
		The first three culumants are mean, variance and third-order central moment. To simplify notation, we denote the mean, variance and third-order central moment of element $\vecElIdx\in[\numVecEl]$ for mixture component $\cmpIdx \in[\numCmp]$ by $\elCmpExp{\cmpIdx}$, $\elCmpVar{\cmpIdx}$ and $\elCmpThrdCenMom{\cmpIdx}$, respectively. From \cite[Chapter~24, Section~3]{Johnson1995}, we find
		\begin{equation}
		\label{eq:beta-cum-def}
			\cum{\cumOrd_\vecElIdx}^{(\cmpIdx)}	= \prod_{\cumOrdIdx = 0}^{\cumOrd-1} \frac{\betaMixA+\cumOrdIdx}{\betaMixA+\betaMixB+\cumOrdIdx}
			%\elCmpVar{\cmpIdx}			&= \E[|\cmpIdx]{\p[\vecElIdx]^2} - \Big(\elCmpExp{\cmpIdx}\Big)^2 =\frac{\betaMixA\betaMixB}{\Big(\betaMixA+\betaMixB\Big)^2\Big(\betaMixA+\betaMixB+1\Big)},\label{eq:beta-mix-def-entry-var}\\
%			\elCmpVar{\cmpIdx}			&\frac{\Big(\betaMixA+1\Big)}{den}\\
%			\elCmpThrdCenMom{\cmpIdx} 	&= \E[|\cmpIdx]{\p[\vecElIdx]^3} - 3\elCmpVar{\cmpIdx}\elCmpExp{\cmpIdx}+2\Big(\elCmpExp{\cmpIdx}\Big)^3
		\end{equation}
		for $\cumOrd\in[3]$. Additionally, denote the mixture component expectation vector by $\vecCmpExp = \Big[\elCmpExp[1]{\cmpIdx}, \dots, \elCmpExp[\numVecEl]{\cmpIdx}\Big]^\top$ and the vector of third cumulants $\vecCmpThrdOrdCenMom = \Big[\elCmpThrdCenMom[1]{\cmpIdx}, \dots, \elCmpThrdCenMom[\numVecEl]{\cmpIdx}\Big]^\top$.
		
		Since the $\p[\vecElIdx]$ are independently distributed, the component covariance matrices $\vecCmpCov$ are diagonal. We additional constrain the model parameters $\betaMixA, \betaMixB \forall\, \vecElIdx \in[\numVecEl]$ such that $\cmpVar\coloneqq \elCmpVar[1]{\cmpIdx} = \dots = \elCmpVar[\numVecEl]{\cmpIdx}$ per component $\cmpIdx\in[\numCmp]$ and thus $\vecCmpCov = \cmpVar\mathbf{I}_{\numVecEl\times\numVecEl}$, where $\mathbf{I}_{\numVecEl\times\numVecEl}$ is the $\numVecEl\times\numVecEl$ identity matrix. This is similar to the spherical covariance assumption in \cite{Hsu2012} and we will hence refer to data following this model as multivariate \textit{spherically beta distributed data}.

		Besides the component-wise quantities, we define the mixture averages of mean, variance and third-order central moment as $\vecExp = [\elExp[1], \dots, \elExp[\numVecEl]]^\top = \sum_{\cmpIdx = 1}^\numCmp\cmpWgt\vecCmpExp$, $\avVar = \sum_{\cmpIdx = 1}^\numCmp \cmpWgt\cmpVar$ and $\avThrdOrdCenMom= [\avElCmpThrdCenMom[1], \dots, \avElCmpThrdCenMom[\numVecEl]]^\top=\sum_{\cmpIdx = 1}^\numCmp\cmpWgt\vecCmpThrdOrdCenMom $.
		The mixture covariance matrix is $\vecCov = \E{(\pvec-\vecExp)(\pvec-\vecExp)^\top}$.
		
		%Finally, we define $\qvec = \big[\q[1], \dots, \q[\numVecEl]\big]^\top$ with $\q = \p[\vecElIdx] - \E{\p[\vecElIdx]}$ as the centered data vector.
	\subsection{Relations between the moments and the mixture parameters}
	\label{sec:sMoM_theo-pop-mom-rel}
		Since \cite[Condition~1]{Hsu2012} is also required for the \gls{smom} estimator to work on spherically beta distributed data, we repeat it for the sake of completeness. 
		\begin{cond}
		\label{cond:1}
			The component expectation vectors $\vecCmpExp$ span a $\numCmp$-dimensional subspace and the entries of $\cmpWgtVec$ are strictly positive. 
		\end{cond}
		The following theorem is the sperical beta data equivalent of Theorem~1 from \cite{Hsu2012}.
		\begin{theo}
		\label{theo:smom}
			Under Condition~\ref{cond:1}, the average variance $\avVar = \sum_{\cmpIdx = 1}^\numCmp \cmpWgt\cmpVar$ is the smallest eigenvalue of $\vecCov$. With $\noiseEigVec \in \mathbb{R}^\numVecEl$ any unit eigenvector of eigenvalue $\avVar$, we define
			\begin{align*}
				\firstPopSMoM 	&= \E{\pvec \Big(\noiseEigVec^\top\big(\pvec-\vecExp\big)\Big)^2},\\ %- \noiseEigVec\odot\noiseEigVec\odot\avThrdOrdCenMom \\
				\secondPopSMoM 	&= \E{\pvec\otimes\pvec} - \avVar\mathbf{I},\\
				\thirdPopSMoM 	&= \E{\pvec\otimes\pvec\otimes\pvec}-\sum_{\vecElIdx = 1}^{\numVecEl}\big(\firstPopSMoM\otimes \baseVec\otimes\baseVec\\ &\qquad+\baseVec\otimes\firstPopSMoM\otimes\baseVec+\baseVec\otimes\baseVec\otimes\firstPopSMoM\big),
			\end{align*}
			with $\firstPopSMoM \in\mathbb{R}^{\numVecEl}$, $\secondPopSMoM \in \mathbb{R}^{\numVecEl\times\numVecEl}$, $\thirdPopSMoM\in\mathbb{R}^{\numVecEl\times\numVecEl\times\numVecEl}$ and the tensor product $\otimes$.
			These observable quantities are related to the population parameters through
			\begin{align*}
				\firstPopSMoM  	&= \firstPopSMoMTheo + \firstPopSMoMErr,\\
				\secondPopSMoM	&= \sum_{\cmpIdx = 1}^\numCmp\cmpWgt\vecCmpExp\otimes\vecCmpExp \coloneqq \secondPopSMoMTheo,\\
				\thirdPopSMoM	&= \thirdPopSMoMTheo + \thirdPopSMoMErr, \\
			\end{align*}
			where we distinguish between the terms depending on the mixture model defining parameters, i.e., the weights $\cmpWgt$, means $\vecCmpExp$ and variances $\cmpVar$,
			\begin{align*}
				\firstPopSMoMTheo 	&= \sum_{\cmpIdx = 1}^\numCmp\Big(\cmpWgt\cmpVar\vecCmpExp\Big) \\
				\thirdPopSMoMTheo 	&= \sum_{\cmpIdx = 1}^\numCmp\big(\cmpWgt\vecCmpExp\otimes\vecCmpExp\otimes\vecCmpExp\big)
			\end{align*}
			and the terms depending on the average third cumulant $\avThrdOrdCenMom$,
			\begin{align*}
				&\firstPopSMoMErr 		= \vphantom{\sum_{\cmpIdx = 1}^\numCmp}\noiseEigVec\odot\noiseEigVec\odot\avThrdOrdCenMom\qquad\qquad\qquad\qquad\thirdPopSMoMErr	= \thirdPopSMoMErrThird - \thirdPopSMoMErrFirst,
			\end{align*}
			where $\odot$ denotes the Hadamard product and
			\begin{align*}
				\thirdPopSMoMErrThird	= \sum_{\vecElIdx = 1}^\numVecEl&\Big(\avElCmpThrdCenMom\,\baseVec\otimes\baseVec\otimes\baseVec\Big)\\
				\thirdPopSMoMErrFirst	= \sum_{\vecElIdx = 1}^\numVecEl&\Big(\firstPopSMoMErr\otimes\baseVec\otimes\baseVec \\
				&+ \baseVec\otimes\firstPopSMoMErr\otimes\baseVec + \baseVec\otimes\baseVec\otimes\firstPopSMoMErr\Big).
			\end{align*}
		\end{theo}
		\begin{proof}
			See Appendix~\ref{apx:smom-theo}.
		\end{proof}
		\begin{cor}
			\label{cor:smom1}
			Asymptotically for large $\numVecEl$, $\firstPopSMoM$ converges to $\firstPopSMoMTheo$ in the \gls{mse} sense. Hence, for larger $\numVecEl$, $\firstPopSMoM\approx\firstPopSMoMTheo$.
		\end{cor}
%		\begin{cor}
%		\label{cor:smom1}
%			Asymptotically, as $\numVecEl$ grows, terms depending on $\avThrdOrdCenMom$ in $\firstPopSMoM$ are expected to vanish and thus
%			\begin{equation*}
%				\lim\limits_{d\rightarrow\infty} \E{\firstPopSMoMErr} = \mathbf{0}_{\numVecEl}, \qquad	\lim\limits_{d\rightarrow\infty} \E{\thirdPopSMoMErrFirst} = \mathbf{0}_{\numVecEl\times\numVecEl\times\numVecEl}.
%			\end{equation*}
%		\end{cor}
		\begin{proof}
			See Appendix~\ref{apx:smom-conv}.
		\end{proof}
		The \gls{smom} estimator from \cite{Hsu2012} depends on $\thirdPopSMoMTheo$ through $\thirdPopSMoMTheoVec{\eta} = \sum_{\vecElIdx_1 = 1}^\numVecEl\sum_{\vecElIdx_2 = 1}^\numVecEl\sum_{\vecElIdx_3 = 1}^\numVecEl\big[\thirdPopSMoMTheo\big]_{\vecElIdx_1, \vecElIdx_2, \vecElIdx_3}[\boldsymbol{\eta}]_{\vecElIdx_3}\baseVec[\vecElIdx_1]\!\otimes\baseVec[\vecElIdx_2]$, where $\boldsymbol{\eta} = [\eta_1, \dots, \eta_\numVecEl]^\top$ is a vector chosen uniformly at random from the unit sphere in $\mathbb{R}^\numVecEl$. Similarly, be $\thirdPopSMoMVec{\eta} = \sum_{\vecElIdx_1 = 1}^\numVecEl\sum_{\vecElIdx_2 = 1}^\numVecEl\sum_{\vecElIdx_3 = 1}^\numVecEl\big[\thirdPopSMoM\big]_{\vecElIdx_1, \vecElIdx_2, \vecElIdx_3}{\eta}_{\vecElIdx_3}\baseVec[\vecElIdx_1]\!\otimes\baseVec[\vecElIdx_2]$. Note, that $\thirdPopSMoMTheoVec{\eta}, \thirdPopSMoMVec{\eta} \in\mathbb{R}^{\numVecEl\times\numVecEl}$.
		\begin{cor}
		\label{cor:smom2}
			$\thirdPopSMoMVec{\eta}$ is an unbiased estimator for $\thirdPopSMoMTheoVec{\eta}$ and the asymptotic \gls{mse} $\lim\limits_{d\rightarrow\infty}\E{\big|\big|\thirdPopSMoMVec{\eta}-\thirdPopSMoMTheoVec{\eta}\big|\big|_F^2}$ is negligibly small. Hence, for larger $\numVecEl$, $\thirdPopSMoMVec{\eta}\approx\thirdPopSMoMTheoVec{\eta}$.
		\end{cor}
%		\begin{cor}
%		\label{cor:smom2}
%			Asymptotically, as $\numVecEl$ grows, 
%			\begin{equation*}
%				\lim\limits_{d\rightarrow\infty}\E{\thirdPopSMoM(\eta)} = \E{\thirdPopSMoMTheo(\eta)}.
%			\end{equation*}
%		\end{cor}
		\begin{proof}
			See Appendix~\ref{apx:smom-conv}.
		\end{proof}		
	\subsection{The proposed spectral method of moments estimator}
	\label{sec:prp-smom}
		Theorem~\ref{theo:smom} and Corollaries~\ref{cor:smom1} and \ref{cor:smom2} enable the development of an \gls{smom} estimator for spherically beta distributed data in combination with \cite[Theorem~2]{Hsu2012}, if $\numVecEl$ is large. Our simulation results suggest that a relatively small $\numVecEl$ is often sufficient. The proposed estimation algorithm for spherically beta distributed data, which we refer to as \learnSB~in what remains, is summarized in Alg.~\ref{alg:learnSB}. Simulation results demonstrating its effectiveness are provided in Sec.~\ref{sec:sim-res}. We observe a set of realizations $\pvecSet = \big\{\pvec_{m}\big\}_{m\in[\numVecObs]}$ of random vector $\pvec$ whose elements are distributed according to the model introduced in Sec.~\ref{sec:sMoM_mv-sph-beta-data}. $\hat{\theta}$ denotes an estimate of a parameter $\theta$ and $\mathbf{X}^\dagger$ denotes the Moore-Penrose inverse of a matrix $\mathbf{X}$.
		\begin{algorithm}
		\caption{\learnSB: The proposed \gls{smom} estimator}
		\label{alg:learnSB}
			\hspace*{\algorithmicindent} \textbf{Input}: $\pvecSet = \big\{\pvec_{\tlIdx}\in\mathbb{R}^{\numVecEl}\,|\,\tlIdx = 1, \dots, \numTls\big\}$, $\numCmp$\\
			\hspace*{\algorithmicindent} \textbf{Output}: $\cmpWgtVecEst\in\mathbb{R}^\numCmp$, $\Big\{\betaMixAEst, \betaMixBEst\Big\},\forall\,\vecElIdx\in[\numVecEl],\forall\,\cmpIdx\in[\numCmp]$
			\begin{algorithmic}[1]
				\State Randomly partition $\pvecSet$ into $\big\{\!\pvecSetOne,\pvecSetTwo\,\big|\,|\pvecSetOne| = |\pvecSetTwo|, \pvecSetOne\,\cap\,\pvecSetTwo = \emptyset\!\big\}$
				\State Compute $\vecExpEstSet{\mathcal{S}} = {|\mathcal{S}|}^{-1}\sum_{\pvec\in\mathcal{S}}\pvec, \mathcal{S} = \pvecSetOne, \pvecSetTwo$
				\State Find ${}_{\mathcal{S}}\hat{\vecCov} = {|\mathcal{S}|}^{-1}\big(\sum_{\pvec\in\mathcal{S}}\pvec\pvec^\top\big)-\vecExpEstSet{\mathcal{S}}\vecExpEstSet{\mathcal{S}}^\top, \mathcal{S} = \pvecSetOne, \pvecSetTwo$
				\State Determine $\avVarEstSet{\mathcal{S}}$, the $\numCmp$-th largest eigenvalue of ${}_{\mathcal{S}}\hat{\vecCov}$  and $\noiseEigVecEst{\mathcal{S}}$, its corresponding eigenvector, $\mathcal{S} = \pvecSetOne, \pvecSetTwo$
				\State Find $\firstPopSMoMEst{\mathcal{S}} = |\mathcal{S}|^{-1}$ $\sum_{\pvec\in\mathcal{S}}\pvec\Big(\noiseEigVecEst{\mathcal{S}}\big(\pvec-\vecExpEstSet{\mathcal{S}}\big)^2\Big), \mathcal{S} = \pvecSetOne, \pvecSetTwo$
				\State Compute the best rank-$\numCmp$ estimate of $\secondPopSMoMTheo$,
				\begin{equation*}
					\secondPopSMoMTheoEst = \arg\min_{\mathbf{X}\in\mathbb{R}^{\numVecEl\times\numVecEl}|\mathrm{rank}(\mathbf{X})\leq\numCmp}\big|\big|{}_{\pvecSetOne}\hat{\vecCov}-\mathbf{X}\big|\big|_2.
				\end{equation*}
				\State Find $\U\in\mathbb{R}^{\numVecEl\times\numCmp}$, the left singular vectors of $\secondPopSMoMTheoEst$
				\State Compute $\W = \U\big(\U^\top\secondPopSMoMTheoEst\U\big)^{\dagger\frac{1}{2}}\in\mathbb{R}^{\numVecEl\times \numVecEl}$ and $\B = \U\big(\U^\top\secondPopSMoMTheoEst\U\big)^{\frac{1}{2}}\in\mathbb{R}^{\numVecEl\times \numVecEl}$
				\State Compute $\thirdPopSMoMEst = |\pvecSetTwo|^{-1}\Big(\sum_{\pvec\in\pvecSetTwo}\pvec\otimes\pvec\otimes\pvec\Big) - \sum_{\vecElIdx = 1}^{\numVecEl}\Big(\firstPopSMoMEst{\pvecSetTwo}\otimes \baseVec\otimes\baseVec+\baseVec\otimes\firstPopSMoMEst{\pvecSetTwo}\otimes\baseVec+\baseVec\otimes\baseVec\otimes\firstPopSMoMEst{\pvecSetTwo}\Big)$
				\For{$t \in [T]$}
				\State Select $\boldsymbol{\eta}_t\in\mathbb{R}^\numVecEl$ uniformly at random from the unit sphere in $\mathbb{R}^\numVecEl$ and define $\boldsymbol{\theta}_t = \W\boldsymbol{\eta}_t$
				\State Find $\W^\top\!\thirdPopSMoMEstVec{\boldsymbol{\theta}_t}\W\!\in\!\mathbb{R}^{\numCmp\!\times\!\numCmp}$, where $\forall\,\cmpIdx_1, \cmpIdx_2\!\in[\numCmp]$,
				\begin{equation*}
					\Big[\W^\top\thirdPopSMoMEstVec{\boldsymbol{\theta}_t}\W\Big]_{\cmpIdx_1, \cmpIdx_2}=\sum_{\vecElIdx_1 = 1}^\numVecEl\sum_{\vecElIdx_2 = 1}^\numVecEl\sum_{\vecElIdx_3= 1}^\numVecEl[\W]_{\vecElIdx_1, \cmpIdx_1}[\W]_{\vecElIdx_2, \cmpIdx_2}[\boldsymbol{\theta}_t]_{\vecElIdx_3}
				\end{equation*}
				\State Determine all (eigenvalue, eigenvector) pairs $\Big(\lambda^{(\cmpIdx)}_t, \mathbf{u}^{(\cmpIdx)}_t\Big), \cmpIdx\in[\numCmp]$, of $\W^\top\thirdPopSMoMEstVec{\boldsymbol{\theta}_t}\W$
				\EndFor
				\State Find $t^\ast = \arg_{t\in[T]}\max\Big(\min_{\cmpIdx_1, \cmpIdx_2\in[\numCmp]}\Big(\Big\{\big|\lambda^{(\cmpIdx_1)}_t-\lambda^{(\cmpIdx_2)}_t\big|:\cmpIdx_1\neq \cmpIdx_2\Big\}\cup\Big\{\big|\lambda^{(\cmpIdx_1)}\big|\Big\}\Big)\Big)$
				\State Compute $\vecCmpExpEst = \Big(\boldsymbol{\eta}_t^\top\mathbf{u}^{(\cmpIdx)}_{t^\ast}\Big)^{-1}\lambda^{(\cmpIdx)}_{t^\ast}\B\mathbf{u}^{(\cmpIdx)}_{t^\ast}$, $\cmpIdx \in[\numCmp]$
				\State Determine $\cmpWgtVecEst = \Big[\vecCmpExpEst[1],\dots, \vecCmpExpEst[\numCmp]\Big]^\dagger\vecExpEstSet{\pvecSetOne}$, $\cmpIdx\in[\numCmp]$
				\State Find $\cmpVarEst\!=\!\frac{1}{\cmpWgtEst}\baseVec[\cmpIdx]^\top\bigg(\Big[\vecCmpExpEst[1],\dots, \vecCmpExpEst[\numCmp]\Big]^\dagger\!\firstPopSMoMEst{\pvecSetOne}\!\bigg)$, $\cmpIdx \in\numCmp$
				\State Obtain $\big\{\betaMixAEst, \betaMixBEst\big\},\forall\,\vecElIdx\in[\numVecEl],\forall\,\cmpIdx\in[\numCmp]$ by inserting the $\vecCmpExpEst$ and $\cmpVarEst$ into Eq.~\eqref{eq:beta-cum-def}
			\end{algorithmic}
		\end{algorithm}		 
		
		The split of $\pvecSet$ into two sets $\pvecSetOne$ and $\pvecSetTwo$ in Alg.~\ref{alg:learnSB} is necessary to prevent distortion of the resulting estimates by correlation introduced due to estimation of $\firstPopSMoM, \thirdPopSMoM$ and $\secondPopSMoM$ from the same data.
		
		In \cite{Hsu2012}, the authors select $T$ such that a specific level of accuracy in the estimated model parameters is guaranteed. In this work, we rely on the approximations $\firstPopSMoM$, $\secondPopSMoM$ and $\thirdPopSMoM$, hence, selection of $T$ according to the criterion in \cite{Hsu2012} might not guarantee a specific level of accuracy. Since typical values of $T$ are small single to double digit positive integers, we propose to simply stick to a fix value, e.g. $T=20$.

==> sections/sim-res_sgl-col.tex <==
\section{Simulation Results}
\label{sec:sim-res}
		\begin{figure}
			\centering
			\begin{subfigure}{.24\textwidth}
				\centering
				\includegraphics[scale=0.45]{figures/sc19_hom_sen_det_pat.pdf}
				%\caption{\gls{fdr}}
				\caption{Detection pattern}
			\end{subfigure}
			\begin{subfigure}{.24\textwidth}
				\centering
				\includegraphics[scale=0.487]{figures/sc19_hom_sen_lfdr.pdf}
				\caption{Interpolated \gls{lfdr}'s}
			\end{subfigure}
			\caption{Example for Sc.~B, Cnfg.~2. In a), the \gls{fdr} threshold is set to $\fdrThr=10\%$. Green, red and gray indicate true, false and missed discoveries. Boxes mark sensor locations. The interpolated \gls{lfdr}'s of b) are discussed in Sec.~\ref{sec:sim-res_spa-ipl}.}
			\label{fig:ex-fd-lfdr}
			\vspace{-13pt}
		\end{figure}
	We evaluate the performance of our proposed method on simulated radio frequency electromagnetic field data. The observed signals are simulated by the nonuniform sampling method from \cite{Cai2003}, which models the propagation of radio waves in a 2D spatial area with path loss and shadow fading \cite{Molisch2012}. The observations are subject to additive white Gaussian sensor noise. If the power of the received signal is below the noise floor, this sensor is classified as located in the true null region $\nulReg$. In our simulations, we alter the sensor noise power for different scenarios to obtain different sizes $|\altReg| = 1-\nulFrc$ of the region of interest. %To obtain the ground true null and alternative regions $\HNul$ and $\HAlt$, we clip the signal below a certain The \gls{snr} is chosen such that the true desired alternative region To obtain the ground true null and alternative regions $\nulReg$ and $\altReg$, we clip the signal below a scenario-dependent threshold

	For simplicity, the sensor \pval s are computed from signal energies. This facilitates the analysis of the results, since its known distributions under null and alternative hypotheses allow for benchmarking the \gls{lfdr} estimation techniques against the true \gls{lfdr}'s. Also, it offers a simple way to simulate a heterogeneous sensor network by alternating the number of measurements $\numSam$ at different nodes. In practice, any type of sufficient test statistic could be deployed at the sensor level.

	We evaluated our method for a variety of simulated propagating radio wave fields in different environments and sensor network configurations. We discuss results for three scenarios typical for radio frequency sensing. %The spatial area of interest is a square of $100\times 100$ pixels, i.e., the total number of pixels is $\numPx=10\,000$.
	The monitored area is discretized by a grid of $100 \times 100$ spatial elements for all scenarios and the results are averaged over $200$ independent Monte Carlo runs, unless stated otherwise. The sources are placed at random locations, i.e., the fraction $\nulFrc$ of grid points in the null region varies slightly from run to run.
	%\textbf{Sc.~A}: A single source in an urban environment. The average relative size of $\altReg$ is $70\%$. This scenario is moderately challenging, since many of the pixels in the alternative region $\altReg$ are exposed to a strong signal. % are exposed for the \zval-based competitors, since many of the observed \zval s stem from the tail of the alternative \gls{pdf} $\altZPdf$ which facilitates its estimation.  %A large number of pixels is under the influence of a single source, i.e., the received signal power is large at many locations in the alternative region. Hence, many observations stem from the tails of the alternative \zval~distribution $\altZPdf$, which facilitates its estimation.

	\textbf{Sc.~A}: Five sources located in a suburban environment covering on average $1-\nulFrc \approx 55\%$ of grid points.
	
	\textbf{Sc.~B}: Eight sources located in a suburban environment covering on average $1-\nulFrc \approx 34\%$ of grid points. %More sources cover less pixels than in Sc.~A, i.e., the observation area in Sc.~B is larger and the spectral resolution of the grid is lower.
	
	 % This scenario is more challenging for the competitors than Sc.~A, since the pixels in the alternative region $\altReg$ are exposed to a weaker signal. The corresponding local summary statistics are hence less distinct from what would be expected in $\nulReg$. %.Many of the observed \zval s stem from $\altZPdf$, but the tails are less pronounced. %A large number of pixels is under the influence of the sources, but due to the propagation model,  since a significant amount of \pval s is generated under $\HAlt$. In contrast to Thus, the alternative a large the joint \gls{pdf} i.e., the 
	\textbf{Sc.~C}: Two sources in a suburban environment covering on average $1-\nulFrc\approx 10\%$ of grid points.
	
	{Sc.~C} is particularly challenging, regardless of the deployed method. Only a small proportion of test statistics provide information on the shape of the alternative component $\altPPdf$.%In addition, a small region of interesting/different/anomalous behavior $\altReg$ makes violations of the nominal \gls{fdr} level more likely, if individual \gls{lfdr}'s of locations in $\nulReg$ are underestimated. 
	
	We investigate three different sensor network configurations.
	
	\textbf{Cnfg.~1}: $\numSen = 10\,000$ identical sensors with $\numSam=256$. Decisions are only made at sensor locations, i.e., no interpolation of decision statistics. This is the classic \gls{mht} problem.
	%\textbf{Cnfg.~1}: Fully loaded. Each grid point hosts a sensor. This configuration of the sensor network is unrealistic in practice, but corresponds to the classic \gls{mht} setting where each hypothesis test is based on a local summary statistic.

	\textbf{Cnfg.~2}: $\numSen=300$ identical sensors with $\numSam = 256$, homogeneously distributed across the monitored area. The tests at the sensors are based on local summary statistics, but in between sensors, the \gls{lfdr}'s are interpolated.
	
	\textbf{Cnfg.~3}: $\numSen_1=170$ sensors with $\numSam_1= 256$, $\numSen=80$ sensors with $\numSam_2= 512$ and $\numSen_3=50$ sensors $\numSam_3 = 1024$, all types homogeneously distributed across the monitored area. Decisions in areas between sensors base upon interpolated \gls{lfdr}'s.
	
	\textbf{Competitors}: We compare our method to a variety of widely used \gls{lfdr} estimators. We deploy the classic \gls{bum} model-based \gls{mle} approach from \cite{Pounds2003}. We also show results obtained with \gls{lm} as proposed by Efron \cite{Efron2010}. \Gls{lm} which approximates the \zval~\gls{pdf} by an exponential family model, fitted to the data using Poisson regression. In addition, \gls{pr} \cite{Newton2002, Martin2011} is applied, which computes the alternative \zval~\gls{pdf} by estimating the density of the mean shift of \zval s from locations in $\altReg$. Predictive recursion has recently \cite{Scott2015, Martin2018, Tansey2018} gained considerable attention in \gls{lfdr} estimation, due to its high accuracy and comparably low computation time. Our implementation of \gls{pr} follows \cite[Appendix~A]{Scott2015}. Finally, we include a standard \gls{gmm}. We do not consider methods whose computational complexity prevents scaling to large-scale sensor networks, as kernel density \gls{lfdr} estimators \cite{Robin2007}.
%	\vspace{-5pt}
	\subsection{The classic multiple hypothesis testing problem}
		\begin{figure}
			\begin{subfigure}{.49\textwidth}
				\centering
				\begin{subfigure}{.49\textwidth}
					\centering
					\includegraphics[scale=0.43]{figures/sc21_fdr.pdf}
					%\caption{\gls{fdr}}
				\end{subfigure}
				\begin{subfigure}{.49\textwidth}
					\centering
					\includegraphics[scale=0.43]{figures/sc21_pow.pdf}
					%\caption{Detection Power}
				\end{subfigure}
			\caption{Sc.~A}
			\label{fig:sca-cnfg1}
			\end{subfigure}
			\begin{subfigure}{.49\textwidth}
				\begin{subfigure}{.49\textwidth}
					\centering
					\includegraphics[scale=0.43]{figures/sc19_fdr.pdf}
					%\caption{\gls{fdr}}
				\end{subfigure}
				\begin{subfigure}{.49\textwidth}
					\centering
					\includegraphics[scale=0.43]{figures/sc19_pow.pdf}
					%\caption{Detection Power}
				\end{subfigure}
				\caption{Sc.~B}	
				\label{fig:scb-cnfg1}		
			\end{subfigure}
			\centering
			\begin{subfigure}{.49\textwidth}
				\begin{subfigure}{.49\textwidth}
					\centering
					\includegraphics[scale=0.43]{figures/sc18_fdr.pdf}
					%\caption{\gls{fdr}}
				\end{subfigure}
				\begin{subfigure}{.49\textwidth}
					\centering
					\includegraphics[scale=0.43]{figures/sc18_pow.pdf}
					%\caption{Detection Power}
				\end{subfigure}
				\caption{Sc.~C}	
				\label{fig:scc-cnfg1}		
			\end{subfigure}
			\caption{\Gls{fdr} and detection power for all scenarios and a sensor network composed of $N=10\,000$ nodes. Inference is only performed at the sensor locations (Cnfg.~1). The \gls{fdr} is strictly controlled for all scenarios by all methods except \gls{lm}. Among the \gls{fdr} controlling methods, ours provides the highest power in Sc.~A, ~B. In Sc.~C, where $\altReg$ contains only a small fraction of all nodes, \gls{pr}'s power is slightly higher.}
			\label{fig:cngf1}
			\vspace{-13pt}
		\end{figure}
		The results for Cnfg.~1 are shown in Fig.~\ref{fig:cngf1}. \Gls{lm} faces stability issues due to the heavy one-sided tail of $\mixZPdf$ when the relative size of the true null region $\nulFrc = |\nulReg|/\numSen$ increases. All other applied methods meet the nominal \gls{fdr} level for all scenarios. We benchmark by the detection results obtained when using the (in practice unknown) true \gls{lfdr}'s. A higher detection than with the true \gls{lfdr}'s can only be achieved, if the respective method violates the nominal \gls{fdr} level.
		For our proposed method, we show results for two variants. For \gls{lfdr}-\gls{smom}${}_s$, the \pval~vectors are formed by subdividing the grid into square tiles of spatially close grid points. For \gls{lfdr}-\gls{smom}${}_r$, the $\{\pPx[\senIdx]\}_{\senIdx\in[\numSen]}$ are randomly partitioned into subsets.

		The results underline that our proposed multivariate \pval~vector probability density model is very flexible. Even if the \pval~subsets are formed at random, the method finds a parametrization such that the individual components have equal variance (Proposition~\ref{prop::model}). This confirms that Assumption~\ref{ass:same-var} can be relaxed in practice.
		For the remainder of this Section, we stick to the conceptually simpler random partitioning and label results obtained with randomly formed \pval~vectors by \textit{\gls{lfdr}-\gls{smom}}.
		
		The traditional \gls{bum} method controls the \gls{fdr}, but exhibits a low detection power in all scenarios, as does \gls{gmm} for larger interesting regions. \gls{pr} performs best by a small margin when the relative size of the alternative region is very small (Sc.~C), but our proposed method achieves the largest detection power in Sc.~A and Sc.~B. Thus, \gls{lfdr}-\gls{smom} provided the best or very close to the best results in all of the considered scenarios.
		
		\begin{figure}
			\centering
			\begin{subfigure}{.35\textwidth}
				\centering
				\includegraphics[scale=0.45]{figures/sc19_fdr_over_size.pdf}
				\caption{\gls{fdr}}
			\end{subfigure}
			\begin{subfigure}{.2\textwidth}
				\centering
				\begin{subfigure}{\textwidth}
					\centering
					\includegraphics[scale=0.45]{figures/sc19_runtimes.pdf}
				\end{subfigure}
				\begin{subfigure}{\textwidth}
					\centering
					\includegraphics[scale=0.45]{figures/sc19_rel_runtimes.pdf}
				\end{subfigure}
				\caption{Execution time}
				\label{fig:rt-b}
			\end{subfigure}	
			\caption{\Gls{fdr}s and run times with increasing sensor network size for \gls{lfdr}-\gls{smom} vs. the best competitor (\gls{pr}).}
			\label{fig:rt}
			\vspace{-10pt}
		\end{figure}
	\vspace{-7pt}
	\subsection{Computational demands as the network size increases}
		In Fig.~\ref{fig:rt}, we compare the best competitor, \gls{pr}, to our proposed method for different sizes of the sensor network $N$ and $1\,000$ \gls{mc} runs. We obtained almost identical results for all scenarios and hence show only those for Sc.~B. Again, inference is only performed at the sensor locations. Both, our method and \gls{pr}, are subject to transient effects when the number of nodes is small. This was to be expected, as fitting a heavy-tailed distribution with such a low number of data points is challenging. Yet, the obtained \gls{fdr}s are close to the nominal level also for the smallest considered network sizes $\numSen$. As $\numSen$ grows, the nominal and empirical \gls{fdr} for \gls{lfdr}-\gls{smom} coincides almost perfectly. Hence, \gls{lfdr}-\gls{smom} is more efficient in exploiting all permitted false positives than \gls{pr}, which results in a larger detection power (plot not shown). The comparison of the average execution time per Monte Carlo run in Fig.~\ref{fig:rt-b} illustrates, that our method is considerably faster than \gls{pr} as $N$ increases. The upper plot shows that the execution time for both methods grows approximately linearly. For a small number of sensors, the runtimes of \gls{lfdr}-\gls{smom} and \gls{pr} are almost identical, but our method scales significantly better for larger sensor networks. At $N=10\,000$, \gls{lfdr}-\gls{smom} is more than five times faster. Both methods were run in Python 3.8.3 on an AMD Ryzen~9 3900X 12-Core CPU.
		
		While \gls{lfdr}-\gls{smom} often provides the highest detection power, it also outperforms its strongest competitor significantly in terms of computation time for growing $\numSen$. \Gls{lfdr}-\gls{smom} is the best fit for large-scale sensor networks.

	\subsection{Spatial interpolation of \gls{lfdr}'s}
		\label{sec:sim-res_spa-ipl}
		It is of high interest to find the boundaries of the regions associated with interesting, anomalous or different behavior. The \gls{lfdr} values between the sensor locations can be determined through spatial interpolation. This allows for segmenting the observation area into $\nulReg$ and $\altReg$. %Finally, we examine Cnfg.~2 and Cnfg.~3, which involve the interpolation of \gls{lfdr}'s at locations between sensor to divide the entire observation area into null and alternative regions.
		
		An exemplary map of interpolated \gls{lfdr}'s with $\numSen = 300$ identical sensors (Confg.~2). is shown in Fig.~\ref{fig:ex-fd-lfdr}, along the detection pattern for the most commonly used \cite{Efron2010} nominal \gls{fdr} level $\fdrThr = 0.1$. In Tab.~\ref{tab:cnfg-2}, we present the numerical \gls{fdr}s and detection powers  obtained by interpolating the estimated sensor \gls{lfdr}'s. Note, that interpolating the \gls{lfdr}'s is a novel approach and could also be combined with any existing \gls{lfdr} estimator, such as \gls{pr}. %Again, we compare our proposed estimator \gls{lfdr}-\gls{smom} to \gls{pr}.
		
		The \gls{fdr} is controlled at the nominal level, except for the very small $\fdrThr=0.01$. This nominal level is so small, that even the slightest interpolation error can lead to its violation. In this example, \gls{lfdr}'s are computed at only $3\%$ of all grid points, and interpolated at the remaining $97\%$. 	
		These results strongly indicate that the interpolation of \gls{lfdr}'s is a powerful tool to decide between $\HNul$ and $\HAlt$ at locations where no sensor is present and local summary statistics are not available.  
		
		In Cnfg.~3, we considered a heterogeneous sensor network composed of multiple types of sensors with different individual detection capabilities due to varying sensor noise levels. The results in Tab.~\ref{tab:cnfg-3} verify the applicability of our method to heterogeneous sensor networks, i.e., to accommodate various types of sensors into the inference process.
		\begin{table}
			\setlength{\tabcolsep}{5.5pt}
			\centering
			\caption{Sc.~B in Cnfg.~2. The columns indicate different nominal \gls{fdr} levels. The similarity in the empirical values of \gls{fdr} and detection power obtained when using \gls{lfdr}-\gls{smom} or in practice the unavailable true \gls{lfdr}'s as base for the interpolation underline the effectiveness of our method.}
			\begin{tabular}{*{9}{c}}
				& $\fdrThr$& $.01$ & $.05$	& $.1$ 	& $.15$ & $.2$ 	& $.25$ & $.3$\\\toprule
				\multirow{2}{*}{\gls{fdr}}		& \textit{True} & $\mathit{.020}$ & $\mathit{.030}$ & $\mathit{.05}$ & $\mathit{.08}$ & $\mathit{.12}$ 	& $\mathit{.17}$ & $\mathit{.22}$\\
				& \gls{lfdr}-\gls{smom} & $.029$ & $.043$	& $.07$ & $.10$ & $.15$ & $.19$ & $.24$	\\\midrule
				%& \gls{pr} & $.018$ & $.028$ & $.05$ & $.07$ & $.10$ 	& $.14$ & $.18$\\

				
				\multirow{2}{*}{Power}			& \textit{True} & $\mathit{.10}$ & $\mathit{.18}$ & $\mathit{.25}$ & $\mathit{.33}$ & $\mathit{.40}$& $\mathit{.47}$ & $\mathit{.55}$\\
				& \gls{lfdr}-\gls{smom} & $.11$ & $.19$	& $.26$	& $.34$ & $.41$	& $.48$ & $.55$	\\\bottomrule
			%	& \gls{pr} & $.10$ & $.17$	& $.24$	& $.30$ & $.37$	& $.43$ & $.50$\\

			\end{tabular}
			\label{tab:cnfg-2}
			\vspace{-7pt}
		\end{table}
		\begin{table}
			\centering
			\setlength{\tabcolsep}{5.5pt}
			\caption{Sc.~B in Cnfg.~3. The columns indicate different nominal \gls{fdr} levels. Also for a heterogeneous sensor network, the \gls{fdr} is controlled except for the very small $\fdrThr=.01$.}
			\begin{tabular}{*{9}{c}}
				& $\fdrThr$ & $.01$ & $.05$	& $.1$ 	& $.15$ & $.2$ 	& $.25$ & $.3$\\\toprule
				\multirow{1}{*}{\gls{fdr}}		& \gls{lfdr}-\gls{smom} & $.023$ & $.039$	& $.07$ & $.11$ & $.15$ & $.20$ & $.25$\\\midrule
				%& \gls{pr} & $.015$ & $.026$ & $.05$ & $.07$ & $.11$& $.15$ & $.19$\\
				
				\multirow{1}{*}{Power}			& \gls{lfdr}-\gls{smom} & $.15$ & $.24$	& $.33$	& $.42$ & $.49$	& $.56$ & $.63$\\\bottomrule
%				& \gls{pr} & $.14$ & $.22$	& $.30$	& $.38$ & $.45$	& $.52$ & $.59$\\
			\end{tabular}
			\label{tab:cnfg-3}
			\vspace{-10pt}
		\end{table}
%	\subsection{Interpolated local false discovery rates}
%	\subsection{Accuracy and computation time with increasing network size}


==> sections/sta-art.tex <==
\section{State of the Art}
\label{sec:sta-art}
	TODO: Describe how this is currently being done and raise the main issues.

==> sections/sys-mod.tex <==
\section{Local inference model}
\label{sec:loc-inf}
	We wish to infer the state of the observed spatial phenomenon at $\numPx$ locations based on observation data acquired on-site.
	%We wish to infer the state of the observed phenomenon on a regular spatial grid composed of $\numPx$ pixels.
	To this end, a decision between the two states of interest, the \textit{absence} or \textit{presence} of a signal, is to be made for every location $\pxIdx\in[\numPx]$ with coordinates $\crdPx = [\xPx, \yPx]^\top$. In the language of hypothesis testing, we aim to make a decision between the \textit{null hypothesis} $\HNul$ (absence of signal) and the \textit{alternative} $\HAlt$ (presence of signal) at each location. The true state of the field at location $\pxIdx$ be denoted by $\HPx$, $\pxIdx\in\numPx$.
	
	This decision is based on a local summary statistic $\locStPx$. Common choices are \pval s $\locStPx=\pPx$ or \zval s $\locStPx=\zPx = \Phi^{-1}(\pPx)$, $\pxIdx\in[\numPx]$. The \gls{pdf} of $\locStPx$ depends on $\HPx$ and is given as
	\begin{align}
		\mixLocStPdf[\pxIdx] =
			\begin{cases}
				\nulLocStPdf[\pxIdx], 		& \qquad \HPx = \HNul \\
				\altLocStPdfLoc{\locStPx},	& \qquad \HPx = \HAlt
			\end{cases}
	\end{align}
	The statistical properties of $\locStPx$ under the alternative $\HAlt$ differ from location to location. This modeling assumptions attributes to the physics of the problem: If a signal is present at two locations $\pxIdx$ and $r$, it will in general have a different impact on the data collected at those two locations, because the signal characteristics depend on different factors as for example the relative location of the source(s). The distribution under $\HNul$, instead, is identical for all locations at which $\HNul$ is in place.

\section{Large-scale inference model}
\label{sec:ls-inf}
	The set of observed location-wise data $\locStSetPx = \{\locStPx[1], \dots, \locStPx[\numPx]\}$ %\zSetPx = \{\zPx[1], \dots, \zPx[\numPx]\}$
	is composed of summary statistics from two mutually exclusive sets of locations $\setFdNul = \{\pxIdx \in[\numPx]|\HPx = \HNul\}$ and $\setFdAlt = \{\pxIdx \in[\numPx]|\HPx = \HAlt\}$. The proportion of locations at which $\HNul$ is in place be denoted by the \textit{null fraction} $\nulFrc = \frac{|\setFdNul|}{|\setFdNul\,  \cup\, \setFdAlt|}$. The \gls{pdf} of a marginal random variable $\locSt$ representing the statistics in $\locStSetPx$ is
	\begin{align}
		\mixLocStPdf 	&= \nulFrc \nulLocStPdf + (1-\nulFrc) \sum_{\pxIdx \in \setFdAlt}\altLocStPdfLoc{\locSt}		\label{eq:zval-mar-pdf_imprac}\\
						&= \nulFrc \nulLocStPdf + (1-\nulFrc) \altLocStPdf.		\label{eq:zval-mar-pdf_prac}
	\end{align}
	The identification of the members of $\setFdNul$ and $\setFdAlt$ is the goal of this work. Hence, the set membership associations are unknown and a decomposition of $\mixLocStPdf$ as in Eq.~\eqref{eq:zval-mar-pdf_imprac} is not possible. In fact, even if the sets $\setFdNul$ and $\setFdAlt$ were known, estimating the alternative probability distributions $\altLocStPdfLoc{\locSt}\,\forall\pxIdx\,\in\setFdAlt$ would be a challenging task, since we only have access to a single observation per $\locStPx\, \forall\, \pxIdx \in\setFdAlt$.
	
	The more practically relevant model in Eq.~\eqref{eq:zval-mar-pdf_prac} replaces the location-wise alternative \gls{pdf}s by the marginal alternative \gls{pdf} $\altLocStPdf$. Eq.~\ref{eq:zval-mar-pdf_prac} is the two-groups model \cite{Efron2010}, which is sufficient to infer whether $\HNul$ or $\HAlt$ is true for each individual location $\pxIdx = 1, \dots, \numPx$ while controlling the \gls{fdr} below a nominal level $\fdrThr$. In addition, the two-groups model permits to profit from having to make multiple decisions between $\HNul$ and $\HAlt$ at the same time, which we will describe in detail in the next section.

	\subsection{Bayesian and local false discovery rates}
	\label{sec:bfdr-lfdr}
		By \cite[Lemma~2.1]{Efron2010}, the \gls{bfdr} of a set $\rejRegLocSt\subseteq\locStSetPx$, defined as
		\begin{equation}
			\label{eq:bfdr-def}
			\bfdr[\rejRegLocSt] = \frac{\nulFrc \nulLocStCdf[\rejRegLocSt]}{\mixLocStCdf[\rejRegLocSt]},
		\end{equation}
		is an upper bound on the Frequentist \gls{fdr} \cite{Benjamini1995}. $\mixLocStCdf[\rejRegLocSt]$ and $\nulLocStCdf[\rejRegLocSt]$ denote the probability of observing $\rejRegLocSt$ and the probability of observing $\rejRegLocSt$ under $\HNul$, respectively. Hence, selecting a rejection set $\rejRegLocSt$ such that $\bfdr[\rejRegLocSt]\leq \fdrThr$ ensures that the \gls{fdr} is below the nominal level.

		The \gls{bfdr} is the probability that any $\locSt\in\locStSetPx$ is a false discovery. In contrast, the \gls{lfdr} \cite{Efron2001, Efron2005} allows to discriminate between individual statistics, asserts a probability of making a false discovery to an individual location and is defined as
		\begin{equation}
			\label{eq:lfdr-def}
				\lfdr[\locSt] = \frac{\nulFrc \nulLocStPdf}{\mixLocStPdf} = \frac{\nulFrc \nulLocStPdf}{\nulFrc \nulLocStPdf + (1-\nulFrc) \altLocStPdf}.
		\end{equation}
		It is equivalent to the posterior probability of $\HNul$ \cite{Efron2005}. The \gls{lfdr} provides more information than the \gls{bfdr}, since the latter is the expected \gls{lfdr} across a set $\rejRegLocSt$, $\bfdr[\rejRegLocSt] = \E[\locSt\in\rejRegLocSt]{\lfdr[\locSt]}$, but does not allow to discriminate between individual $\locSt \in \rejRegLocSt$. If we were able to compute $\lfdr[\locStPx] \, \forall\, \pxIdx\in[\numPx]$, we could hence perform classical multiple hypothesis testing by rejecting $\HNul$ at the locations of  $\locSt\in\rejRegLocSt$ such that $\bfdr[\rejRegLocSt]\leq \fdrThr$. In addition, we could also provide a probability on how likely we were to make a false discovery if we declared a single $\locSt$ to be alternative.
		
		Estimation of the \gls{bfdr} requires knowledge of $\nulFrc$, $\nulLocStCdf$ and $\mixLocStCdf$, whereas estimation of the \gls{lfdr} relies on $\nulFrc$, $\nulLocStPdf$ and $\mixLocStPdf$. The quantities in the numerators of Eq.~\eqref{eq:bfdr-def} and Eq.~\eqref{eq:lfdr-def} are often straight forward to acquire. Under the null hypothesis, \zval s follow a standard normal distribution, $\nulZCdf= \Phi(\z)$ and $\nulZPdf = \phi(\z)$, whereas \pval s follow a uniform distribution $\nulPPdf$ on $[0, 1]$. The proportion of true null hypotheses $\nulFrc$ is often set to its upper limit $\nulFrc = 1$, to obtain an upwardly biased estimate of the \gls{bfdr}, thereby avoiding the estimation of $\nulFrc$. Overestimation of the \gls{bfdr} leads to a rejection set with a true \gls{fdr} below the nominal level. When deciding in favor of estimating $\nulFrc$ from the data, one needs to be careful not to underestimate its value, which would lead to an underestimation of the \gls{bfdr} and hence a potential violation of the nominal \gls{fdr} level. A variety of methods to conservatively estimate $\nulFrc$ from the data exist, the most frequently utilized approaches were introduced in \cite{Storey2002} and \cite[Chapter~4.5]{Efron2010}. The numerators of the \gls{bfdr} and \gls{lfdr} are more challenging to deal with, since the marginal distribution $\mixLocStCdf$ and density $\mixLocStPdf$ also depend on the unknown characteristics under the alternative. A simple and efficient estimator for a cumulative distribution function $\mixLocStCdf$ is the corresponding \gls{edf} $\mixLocStCdfHat = \frac{\sum_{\pxIdx = 1}^{\numPx}\idc{\locStPx\leq \locSt}}{\numPx}$, where $\idc{\cdot}$ is the indicator function. In contrast, the estimation of the corresponding density $\mixLocStPdf$ requires fitting an unknown density and makes the computation of \gls{lfdr}s far more challenging \cite{Efron2010}.
		
	\subsection{Contextual information}
	\label{sec:con-inf}
		As illustrated in the previous section, \gls{lfdr}s are more meaningful than the \gls{bfdr}, at the price of being more difficult to estimate. In this section, we elaborate on another significant conceptual advantage of \gls{lfdr}s, namely, that they allow to accommodate available contextual information into the inference process. In many applications, the local summary statistics are not the only available information. A prime example is the problem considered in this work: Besides its $\locStPx$, we also know the coordinates $\crdPx$ of location $\pxIdx\in[\numPx]$. Spatial phenomena in general exhibit some form of spatial correlation and hence, the field is expected to be in a similar state at locations close to each other. Thus, one is able to improve the inference quality by taking into account the information on the state of the field available at nearby locations. A neat way of doing so is to make $\nulFrc$ a function of the additional information available for each $\locStPx,\, \pxIdx\in[\numPx]$. This leads to \textit{contextual} \gls{lfdr}s
		\begin{equation}
			\label{eq:lfdr-spa-def}
			\lfdrLoc{\locSt} = \frac{\nulFrcLoc\nulLocStPdf}{\nulFrcLoc\nulLocStPdf + (1-\nulFrcLoc)\altLocStPdf},
		\end{equation}
		where the location index $\pxIdx \in [\numPx]$ indicates the dependency on any available contextual information for location $\pxIdx$. Given that the location-dependent probabilities of $\HNul$, $\nulFrcLoc$, incorporate the additional information available at the other locations in a proper way, the contextual \gls{lfdr} as defined in Eq.~\eqref{eq:lfdr-spa-def} is a more meaningful quantity than the standard \gls{lfdr} as defined in Eq.~\eqref{eq:lfdr-def}. Besides the necessity to incorporate the available location information into $\nulFrcLoc$ in a proper way, the numerator of Eq.~\eqref{eq:lfdr-spa-def} requires a decomposition of $\mixLocStPdf$ into the null and alternative components, which is an even more challenging task than the estimation of $\mixLocStPdf$ required for Eq.~\eqref{eq:lfdr-def}.
		
		In what follows, we will first deal exclusively with the problem of appropriate estimation of the null and alternative components of $\mixLocStPdf$ as defined in Eq.~\eqref{eq:zval-mar-pdf_prac}, before returning to the estimation of spatially-dependent priors $\nulFrcLoc$ in Section XX.


==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}
\usetikzlibrary{shapes.geometric}
% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspamp/.style={shape=regular polygon, regular polygon sides=3,draw,align=center,text depth=0.3em,text height=0.6em,inner sep=0pt,line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}} %,draw,

\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}
\tikzset{dspflow2/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.25 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

